Embedding Recycling for Language Models

Real-world applications of neural language models often involve running many different models over the same corpus. The high computational cost of these runs has led to interest in techniques that can reuse the contextualized embeddings produced in previous runs to speed training and inference of future ones. We refer to this approach as embedding recycling (ER). While multiple ER techniques have been proposed, their practical effectiveness is still unknown because existing evaluations consider very few models and do not adequately account for overhead costs. We perform an extensive evaluation of ER across eight different models (17 to 900 million parameters) and fourteen tasks in English. We show how a simple ER technique that caches activations from an intermediate layer of a pretrained model, and learns task-specific adapters on the later layers, is broadly effective. For the best-performing baseline in our experiments (DeBERTa-v2 XL), adding a precomputed cache results in a >90% speedup during training and 87-91% speedup for inference, with negligible impact on accuracy. Our analysis reveals important areas of future work.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> submissions/TMLR August 2022/1-intro.tex <==
\begin{abstract}

Training and inference with large neural models is expensive.  However, for many application domains, while new tasks and models arise frequently, the underlying documents being modeled remain mostly unchanged.  We study how to decrease computational cost in such settings through {\em embedding recycling (ER):} re-using activations from previous model runs during training or inference. In contrast to prior work focusing on freezing small classification heads for fine-tuning which often leads to notable drops in accuracy, we propose caching an intermediate layer's output from a pretrained model and fine-tuning the remaining layers for new tasks. We show that our method is effective using either fine-tuning for the trainable layers, or parameter-efficient adapters.  For the best-performing model in our experiments, DeBERTa-v2 XL with adapters, we find that our method provides a 100\% speedup during training and an 87-91\% speedup for inference, and has negligible impacts on accuracy averaged across eight tasks spanning text classification and entity recognition in the scientific domain and general-domain question answering.  Further, in experiments with SciBERT, BERT-base, and RoBERTa-large, we show a 100\% speedup during training and a 55-86\% speedup for inference, at only a 0.19-0.23\% reduction in accuracy on average.
%, showing a superior accuracy-efficiency tradeoff to prior QA-specific decomposition techniques.
%Our experiments span eight data sets and five different model sizes, using both standard fine-tuning and parameter-efficient adapters.
Finally, we identify several open challenges and future directions for ER.
% \arman{I think we would benefit from adding one or two more sentences on how our ER approach is different than prior work and explaining the setup on static document collections. We can shorten the results sentences to find space. }


%Training and running large language models is necessary for achieving state-of-the-art performance on a variety of computational tasks. Numerous studies have shown that, generally, larger language models perform better than smaller, more compact models. However, it is ultimately computational expensive at both training and inference time to generate sequence representations for large corpora. Furthermore, for large document datasets that do not change substantially day-to-day, such as the Semantic Scholar (S2) document database, running a new language model requires recomputing the embedding for each document. This can make testing new language models and generating sequence representations for documents computationally prohibitive. 

%To alleviate this problem, we introduce embedding recycling, a technique for storing and reusing previously generated sequence representations for future tasks. Through embedding recycling, we can effectively retrieve a set of precomputed embeddings for various NLP tasks, such as text classification and named-entity recognition (NER), without the need for recomputations. Additionally, by coupling precomputed embeddings with reduced large language models, we can achieve comparable or superior accuracy across several scientific NLP tasks. From our experiments, we have shown that embedding recycling can reduce both training time and inference time in half as well as substantially reduce memory footprint for GPU-based computations. Furthermore, for a variety of different large and compact language models, we have shown that freezing earlier layers in their computational architectures can preserve or improve performance for scientific NLP tasks.

\end{abstract}

\section{Introduction}

Large pretrained language models form the foundation of modern NLP, and continue to push the state-of-the-art on a wide range of natural language processing tasks \citep{devlin2018bert,liu2019roberta,bommasani2021opportunities}.  Larger models tend to offer superior accuracies \citep{kaplan2020scaling}, but also higher  computational costs.  The steep computational cost  associated with large neural language models slows down experimentation, increases financial barriers to the technology, and contributes to global climate change \citep{strubell2019energy, dodge2022measuring}.

We explore how to reduce this computational cost using the simple observation that often, the text we wish to process with a large neural model has already been processed through a model before---and the activations from previous runs may be re-used to speed up the current one.  In many corpora, substantial portions of the text remain relatively fixed over time (e.g. scientific papers, Wikipedia articles, StackExchange posts, financial reports, legal records, etc.).  Further, a number of models for various tasks are run over this text (entity recognition, topic classification, relation extraction, summarization, question answering, and so on).  %Further, individual practitioners often repeatedly train the same large model on the same text e.g. hyperparameter search \arman{This is an interesting use case. If we do hyperparam tuning under ER setting and find optimal ones, do we know if the same hyperparams would be optimal for the original model?}.
Any one of the runs produces a contextualized embedding of the text; and even without task-specific fine-tuning, contextualized embeddings produced by pretrained language models are known to capture syntactic and semantic knowledge about their input texts \citep{goldberg2019assessing,wiedemann2019does,rogers-etal-2020-primer}, which can be useful for a variety of downstream tasks.

We study {\em embedding recycling} (ER), the technique of leveraging activations from previous model runs in order to improve the accuracy and efficiency of future training and inference.  While previous work has explored a similar approach using frozen encoders \citep{du2020general}, it focuses on small classification heads for fine-tuning which lead to drops in accuracy.  By contrast, we experiment with a simple {\em layer-recycling} ER method that stores a cache of the activations from an intermediate layer of a pretrained model, and then starts from those activations when the same input sequence is seen again during fine-tuning or inference.  Layer recycling imposes a small additional time cost the first time a model is run on a text, in order to compute and write the cache. Then, all subsequent runs on the text can start from the pretrained cache, which we show results in substantial increases in throughput for those runs at small or no cost to model accuracy.  This is significant because the number of such subsequent runs can be large in some real-world applications, including when re-training models many times during development, executing many epochs in a training run, or performing inference with many different models over the same corpus \cite{du2020general,Wei2022AFM}.

%The contextualized activations are known to capture syntax and semantics of the text \cite{}, and show .

%The increasingly large models of modern NLP come with a correspondingly large computational cost, which slows down experimentation, increases hardware costs, and .  These costs are exacerbated by the fact that similar models are frequently finetuned on the same corpus; for example, for large document corpora such as Wikipedia articles, StackExchange posts, and academic papers there are many tasks of interest (entity recognition, classification tasks, question answering, and so on) that are often approached by applying different finetunings of the same pretrained model, bearing the full cost of processing the corpus each time.  Additionally, in research settings it is common to retrain the same model on the same data with slightly different hyperparameters to improve results and test the variability of results.  The cost of re-processing the same corpora motivates us to consider ways to re-use past computations to reduce the cost of future tasks.
%  for each of the are often added to but rarely modified, and there are several modeling tasks done on .  f this repetition is the rerunning of models on the AI's Semantic Scholar (S2) document database, a corpus that only changes marginally day-to-day. \arman{This is a very specific dataset. I would just combine this with the next sentence} For any other large document corpus, such as Wikipedia or StackExchange, similar models are reconfigured and run on the same set of documents, generating very similar sequence representations. 


To summarize, we make the following contributions:

\begin{itemize}
    \item We propose embedding recycling as a method for lowering the computational costs of training and inference for language models, and explore two layer recycling methods, one that uses standard fine-tuning and another that uses parameter-efficient adapters.
    \item In experiments across seven models and eight tasks, we show that layer recycling is generally effective.  For the best-performing model on our tasks, DeBERTa-XL with adapters, we find that layer recycling matches performance of the original model while providing a 87-91\% speedup at inference time, and a 100\% speedup at training time.%, achieving a superior accuracy-efficiency tradeoff to prior QA-specific decomposition techniques \cite{cao2020deformer}.  
    %\mike{speedup based on Luca's BERT results in Table \ref{tab:performance}} \mike{Should we also mention sharing across model architectures here?  Didn't want to get too lengthy but that might be important enough to include}
    \item We explore open challenges for embedding recycling and present questions for future work.
    %\item We show that across a variety of large and compact language models, freezing earlier layers in model architectures can preserve or improve performance on scientific NLP tasks while reducing both training and inference time in half. 
    %\item We demonstrate that by coupling embedding recycling with reduced large language models, we can preserve or improve the performance of the large language models while also gaining new improvements to training and inference times.
    %\item Using embedding recycling, we either match or outperform other competitive models, such as Adapter models and distilled models, but also successfully reuse precomputed embeddings to improve training and inference times.
    %\item We explore a variety of real-world scenarios for effectively using embedding recycling to avoid recomputations for large document corpora.
\end{itemize}


==> submissions/TMLR August 2022/2-experiments.tex <==

\section{Related Work}

%Recent work has focused on reducing the computational restrictions for running large language models to improve their applicability. \citet{sajjad2020effect} focused on reducing the network size of large language models, such as BERT, RoBERTa, and XLNet, by dropping layers in pretrained models, while preserving most of the performance gains over more compact models. Additionally, several recent efforts have employed different approaches for freezing layers in large language models, either actively freezing certain parameters while fine-tuning or freezing layers before fine-tuning even begins, to achieve close to fully fine-tuned performance \citep{Lee2019WhatWE, Brock2017FreezeOutAT, Liu2021AutoFreezeAF, Xiao2019FastDL}. Other work explored freezing large language models from training and adding fine-tunable modules, such as Adapters, bias weights, and soft prompts \citep{ding2022delta, houlsby2019parameter, qin2021learning}. 

%While these explored approaches have improved training time for large language models \arman{this is not always the case. E.g., many parameter efficient training methods actually do not decrease training time}, none of them have managed to cut training time while preserving the best performance of these models. Furthermore, none have sought to reuse previously generated sequence representations to boost either training or inference time. \citet{cohan2020specter} introduced the SPECTER API for sharing document representations for future use but our work seeks to reuse representations across tokens, sequences, and documents, allowing us to retrieve an embeddings set for a given task and reducing the need for expensive fine-tuning.

%While previous work on partially-frozen model fine-tuning improves training time by skipping the backward pass of shallow model layers, none of those studies attempt to re-use computation on previously-seen sequences, and therefore they save no computation at inference time and don't eliminate the forward pass from the frozen layers even at training time.  In this work we explore {\em embedding recycling}, a method of speeding up training and inference by storing a cache of the activations from an intermediate layer of a pretrained model and then re-using those activations when the same input sequence is seen again.  Our results are consistent with prior work showing that pretrained models can perform well even when only their deeper layers are fine-tuned, but we additionally show that the intermediate activations of the model can be efficiently cached and retrieved to significantly speed up both training and inference time.



% \subsection{Pretrained Language Models}

% Pretrained language models are first trained on large textual corpora before being fine-tuned for specific downstream tasks. %\citet{peters-etal-2018-deep} \mike{TODO: wording---pretraining+fine-tuning was a thing before ELMo (e.g., Dai and Le 2015, ULMFiT)} was among the first to successfully apply this model training setup through ELMo, which outperformed state of the art models across core NLP tasks, such as sentiment classification, question answering, token classification, and natural language inference. %\citet{devlin2018bert} built upon ELMo by incorporating transformer layers \citep{vaswani2017attention} and creating BERT, a pretrained transformer encoder model.  Other models, such as RoBERTa \citep{liu2019roberta} and XLNet \citep{https://doi.org/10.48550/arxiv.1906.08237}, have expanded on the pretrained transformer model setup by expanding pretraining datasets while improving model architectures.%

Transformer-based pretrained language models (PLMs) are typically first pretrained over a large text corpus and then fine-tuned on a downstream task. Recent work analyzing the structures of neural networks has shown that different layers within transformer models extract different features from textual data.  Studies using canonical correlation analysis have found that the shallower layers tend to converge earlier in training than the deeper layers \citep{raghu2017svcca,morcos2018insights}. \citet{kovaleva2019revealing} observed that the last layers of BERT change the most substantially during fine-tuning, suggesting that earlier layers tend to extract universal features whereas later layers focus on task-specific modeling.% \citet{sajjad2020effect} differentiate between the transformer models and found that RoBERTa and XLNet learn task-specific knowledge earlier in the network compared to BERT.

%Consistent with the idea that task-specific knowledge is primarily learned by later layers, several studies found that earlier layers can be frozen with only a minor degradation in end-task performance.
This tendency of deeper layers to learn task-specific knowledge has led to a variety of work finding that it is often not necessary to train all the layers of a model.  \citet{Lee2019WhatWE} found that only a fourth of the final layers in BERT and RoBERTa need to be fine-tuned to achieve 90\% of the fully fine-tuned performance.  Other work explored adaptive approaches that vary the number of frozen layers over the course of training, approaching or exceeding the performance of fully fine-tuned models while substantially speeding up the training process \citep{raghu2017svcca, Xiao2019FastDL, Brock2017FreezeOutAT}.

Similar to our work, some prior work on dynamic freezing also employed caching mechanisms to eliminate the cost of the forward pass for frozen layers \citep{Liu2021AutoFreezeAF,he2021pipetransformer}.  However, in that work the dynamic choice of how many layers to freeze means that the cached activations are only useful at training time and only for a single task; we propose caching embeddings from the pretrained model, which can then be reused across multiple downstream tasks and applied at inference time as well.


%Of particular relevance to our work is the work of \citet{Liu2021AutoFreezeAF}, a dynamic freezing approach which also caches the activations of the frozen portion of the network to further accelerate training while maintaining task results.  

%Since only a few of the final transformer layers are needed to achieve high performance on downstream tasks, \citet{Lee2019WhatWE} found that only a fourth of the final layers in BERT and RoBERTa need to be fine-tuned to achieve 90\% of their fully fine-tuned performance. Other recent work has sought to develop adaptive systems during fine-tuning to selectively freeze layers and blocks, approaching the performance of fully fine-tuned models while substantially speeding up the fine-tuning process \citep{Liu2021AutoFreezeAF, Xiao2019FastDL, Brock2017FreezeOutAT}. 
%While past studies have shown how freezing or dropping transformer layers can preserve performance gains and cut fine-tuning time, none have successfully matched or improved the performance of fully fine-tuned language models. \mike{What special thing are we doing that makes us match or improve the performance?  If we're doing essentially the same freezing procedure and just using different datasets that work better, I would hesitate to claim that we were successful at the same thing they were unsuccessful at.  Probably should focus on the caching aspect which wasn't really addressed in those works.}

Other recent studies have sought to improve model inference speed by skipping computations in later layers.  \citet{sajjad2020effect} found that for some tasks and PLMs, up to half of the layers can be removed from the model to obtain a 98-100\% speedup at the cost of a 1-3\% drop in task performance.  \citet{kumar2019accelerating} considered approximate caching to skip the deeper layers for inputs that produce similar intermediate layer representations.  Early exit strategies have also been proposed, which allow the model to dynamically decide when to skip later layers \citep{cambazoglu2010early,xin2020deebert}.  In contrast, embedding recycling focuses on eliminating computation of earlier layers rather than later ones, which makes it potentially possible to combine embedding recycling with early exiting.

SkipBERT \citep{wang2022skipbert} combined early exiting with an approach in which cached n-gram embeddings (tri-grams in practice) were used to approximate the intermediate activations of new inputs.  However, SkipBERT only measures latency (with a batch size of 1), targeting the use case where individual new inputs need to be processed quickly.  In embedding recycling, we focus on the case where an entire cached corpus needs to be processed at once, making throughput more important than small-batch latency.  In addition, SkipBERT's approach is only evaluated on BERT-base and only on sentence-level tasks, whereas we demonstrate the generality of embedding recycling across 8 models and 3 task types.
% - more specific case (stronger assumption)
% - more model sizes
% - measure throughput not latency
% - sequence tagging tasks

Precomputing text representations to speed up future processing on the same data is commonly done when creating fixed-size document-level embeddings for use on document-level tasks  \citep{conneau2017supervised,cohan2020specter}; in contrast, we study contextualized {\em token-level} embeddings that can be used for tasks such as named entity recognition (NER) and question answering.  ReadOnce Transformers \citep{lin2021readonce} do consider multi-task variable-length document representations, but do so in the context of "representation+text" style tasks such as question answering, where a cached document representation is paired with a query text at inference time (such as a question or prompt); the approach is pretrained with question answering data and evaluated on QA and summarization, rather than tasks such as text classification or NER where the entire input can be cached.

\citet{du2020general} propose a similar high-level idea to ours in that they do cache general-purpose token-level model representations, trained in a multi-task setting; however, the approach in that work only applies a small MLP to the stored representations and reports a meaningful drop in accuracy (greater than 2\% on average) compared to fully fine-tuned models.  We find that reusing the later layer parameters of a pretrained transformer in addition to the cached activations of prior layers enables us to often essentially match fully fine-tuned model accuracy on average, while decreasing computational cost.  As noted in our experiments, if we instead use small MLPs from a frozen pretrained encoder, we see large drops in accuracy on our tasks. %\mike{We could mention that we do an analysis of real-world speedup as opposed to just using FLOPS (that turns out to matter since we have some overhead to transfer embeddings), but for now I'm omitting it for brevity}

%\mike{TODO?: mention delta-tuning/parameter-efficient methods, although I'm increasingly unsure if that's actually important to include in this section.}
%Another set of work related to pretrained model reuse is delta tuning \citep{ding2022delta}, a class of methods aiming to train only a small number of parameters to adapt a model for a downstream task.  Delta tuning methods include adapters, bias weights, and soft prompts \citep{houlsby2019parameter, qin2021learning}.


%\mike{TODO?: Maybe mention work on reusing attention, e.g. \citep{xiao2019sharing}}
\citet{Wei2022AFM} combine the practices of freezing shallow layers and knowledge distillation to create a multi-task model. However,  they use a two stage process where $12-N$ deep layers are fine-tuned for each individual task keeping $N$ frozen layers. This is followed by distillation of the $N$ layers for further computational gains. We take advantage of the parameter efficient adapter modules \citep{houlsby2019parameter}, and replace this process with a single step of fine-tuning a frozen base model that has adapters attached only to the deeper layers.

%\arman{added the following paragraph}
%Our work also has connections to prior work on utilizing memory and caching earlier hidden states in a sequence within Transformer models (e.g., \cite{grave2016improving,dai2019transformer,rae-razavi-2020-transformers,wu2022memorizing}). These works generally focus on modeling long range context and caching representations of older history in a sequence. In contrast, our work focuses on caching the representations of the entire sequence and using it for new tasks.  
%\arman{end}

%\mike{I like the above but it is missing retrieval methods the reviewer mentioned.  How about the following?}
Our work also has connections to work on memory- and retrieval-augmented language modeling.  Prior work on using memory (e.g., \cite{grave2016improving,dai2019transformer,rae-razavi-2020-transformers,wu2022memorizing}) generally focuses on modeling long range context and caching representations of older history in a sequence, while work on retrieval (e.g., \citep{pmlr-v119-guu20a,karpukhin_etal_2020_dense}) focuses on fetching text from a knowledge base or corpus to serve as additional context.  In both cases, the aim is to use representations of additional text (from earlier in a document or from a knowledge base) to improve modeling of new inputs.  In contrast, our work focuses on caching the representations of an entire sequence to speed up computation for new tasks.
%\mike{end}

%\mike{Some sweeping generalizations were made here in an attempt to improve brevity; also there is a bunch of work in this area and I haven't cited all of it.  So, the paragraph would benefit from a second set of eyes.  It's possible that we could replace it with just some version of the last sentence as a very broad rationale for why we don't cover this space in more depth, but I'd like to be thorough enough to address the reviewer's concerns.}
%\aps{I have edited the last sentence from Mike's original draft. I feel like the last 2 sentences below and Arman's change above can be combined together which should be enough?}
%Embedding recycling is broadly related to retrieval- and memory-augmented language modeling insofar as it stores representations of past inputs which are later retrieved to support future inferences.  Passage-retrieval methods such as REALM \citep{pmlr-v119-guu20a} and DPR \citep{karpukhin_etal_2020_dense} retrieve relevant texts from a knowledge base to augment the information available to a model.  Neural cache models \citep{grave2016improving} and Transformer-XL \citep{dai_etal_2019_transformer} increase the effective context size of models by storing representations of previously-seen text in a document and retrieving them as additional context for subsequent input tokens.  Finally, memory-augmentation methods such as memorizing transformers \citep{wu2021memorizing} and neural turing machines \citep{graves2014neural} allow models to use a differentiable key-value storage as external memory.  However, while all of these approaches focus on  increasing context to improve accuracy for new input text, in ER we aim to reduce computational cost by caching .
%All of these approaches focus on using past computations to improve accuracy by modeling long range context. In contrast, we aim to reduce computation cost by caching and reusing past computations on already seen data.
%Several works augment language models by retrieving text or text embeddings that add relevant information to a given input.  Transformer-XL \cite{} and memorizing transformers \cite{} store representations of previously-seen text to provide additional context for subsequent input chunks.  Other methods, such as REALM \cite{} and DPR \cite{}, retrieve text passages from a knowledge base with which to augment the information available to a model.  However, all of these approaches aim to add information from additional text to improve inference accuracy (but still incur the full cost of the model) for a new input text, whereas in ER we aim to use information from past computations on the same text to reduce computational cost.

\section{Methods}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=\linewidth]{Images/EmbeddingRecycling.png}
%    \caption{Overview of the embedding recycling approach. In the figure, the K-th layer activations are saved for future fine-tuning on downstream tasks, skipping redundant computations of earlier layers in the transformer model.}
%    \label{fig:embedding_recycling}
%\end{figure}

\begin{figure}[t]
%\begin{center}
\centering
%\framebox[0.95\textwidth]{\includegraphics[width=\textwidth]{Images/EmbeddingRecycling.png}}
\fbox{\includegraphics[width=0.5 \textwidth]{Images/EmbeddingRecycling.png}}
%\includegraphics[width=\linewidth]{Images/EmbeddingRecycling.png}
%\end{center}
\caption{Overview of the embedding recycling approach. In the figure, the K-th layer activations are saved for future fine-tuning on downstream tasks, skipping redundant computations of earlier layers in the transformer model.}
\label{fig:embedding_recycling}
\end{figure}

In the transformer architecture \citep{vaswani2017attention}, an input sequence $x$ of length $S$ and dimension $d$ is transformed with a function $F: \mathbb{R}^{S\times d} \rightarrow \mathbb{R}^{S\times d}$ defined by the composition of $N$ transformer layers $F^{(1)}, ... , F^{(N)}$ as follows:

\begin{equation} \label{eq:transformer}
    \texttt{F}^{\ell}(x) = \texttt{LN}(\texttt{FF}^{\ell} (\; x') + x') 
\end{equation}

% \begin{equation} \label{eq:self_att}
%     \texttt{SA}^{\ell}(x) = \texttt{FF}^{\ell} (\; x')
% \end{equation}

\begin{equation} \label{eq:self_att}
    \texttt{x'} = \texttt{LN}\Big(\texttt{MH}^{\ell}(x)+x\Big)
\end{equation}


\noindent where $\texttt{LN}$ is a layer normalization \citep{Ba2016LayerN}, $\texttt{FF}$ is a feed forward network, and $\texttt{MH}$ is the self-attention layer that consists of multiple heads and contextualizes the input sequence vector. The output of each layer is used as input to the next layer. 
\begin{equation}
    h^{\ell+1} = F^{\ell}(h^{\ell})
\end{equation}

Our approach is to cache the output representations $h^{k}\in \mathbb{R}^{S\times d}$ at a certain layer $k$ and reuse them for fine-tuning on a new given task. We refer to this process of caching and reusing the output representations of a layer as {\em layer recycling}. This enables us to reduce the size of the transformer model from $N$ layers to $N-k$ layers, reducing the computational cost during fine-tuning and inference. 

Note that the key requirement of layer recycling is that we first need to process the entire data with the transformer model and cache the representations, so that we could later reuse these representations many times during fine-tuning and inference on new tasks. We experiment with two types of layer recycling approaches as explained next.

% Within the transformer architecture, activations are generated at each transformer layer sequentially before being fed into the next layer in the model. In our within-model approach, we use a \textit{source model} to run over a selected corpus before our experiments, caching the activations for each input locally. During the experiments, a \textit{consumer model} then uses the cached activations for fine-tuning and testing. \arman{Cached activations or hidden states?} Both the source model and the consuming model have the same architecture.

We start with a pretrained transformer $F$ (e.g., BERT) consisting of $F^{(1)}, ..., F^{(k)}, ... , F^{(N)}$ layers. We run the transformer over a corpus $\mathcal{C}$ and cache the output representations of layer $k$ for each instance $c$ in $\mathcal{C}$, i.e., $h^{k}_{c\in\mathcal{C}}$. 
The same transformer model is then used for fine-tuning on new tasks, however, instead of fine-tuning all the layers, we only fine-tune the parameters of the latter $N-k$ layers $F^{(k+1)}, ..., F^{(N)}$. We can either train all of the weights in these layers (we refer to these as {\em reduced models}), or only train adapter modules added on the layers (discussed below). In either case, for the instance $c$ in the dataset $\mathcal{C}$ we simply retrieve and use the previously cached representation $h^{k}_{c\in\mathcal{C}}$ as input to layer $F^{(k+1)}$. This avoids the extra computation through layers $F^{(1)}, ..., F^{(k)}$ but adds a small cost for retrieving the representation from storage (see \autoref{sec:performance_analysis} for efficiency analysis).

\subsection{Adapters}

%The layer recycling methods in our experiments use the standard fine-tuning approach for the remaining layers, creating a new reduced model for each new task.  As model size and the number of tasks increases, it could become expensive to store and communicate the layers for each task.  As a proof of concept experiment we evaluate whether recent parameter-efficient techniques can address this issue.  \citet{houlsby2019parameter} introduce adapter modules as a parameter efficient fine-tuning approach which adds a few extra parameters to the transformer model that are trained, leaving the rest of the architecture frozen. \jon{Add motivation for why parameter-efficient storage isn't the focus (since the storage costs of adapters are much smaller than the cost of storing embeddings) and instead the motivation is improved performance}

In addition to the standard layer recycling, we evaluate whether combining layer recycling with Adapter modules \citep{houlsby2019parameter} can improve performance as compared to fully fine-tuned models. Adapters are typically used to improve the parameter efficiency of finetuning and mitigate the storage costs of large language models. They also enable more sample-efficient fine-tuning and can result in improved fine-tuning performance \citep{karimi-mahabadi-etal-2022-prompt}. Therefore, we investigate whether Adapters can also yield accuracy improvements when used in combination with layer recycling.

Adapter modules contain a down-projection, an up-projection, and a residual connection module: 
$h\leftarrow h+ (f(h\mathbf{W}_{down})\mathbf{W}_{up})$. The adapters are separately inserted after the \texttt{MH} and the \texttt{FF} layers in the transformer architecture (\autoref{eq:self_att}). Further, \citet{Rckl2021AdapterDropOT} experiment with dropping adapters from the lower transformer layers to provide inference time speedup. In our experiments, adapters are added to the latter half of transformer layers in the reduced transformer models. Particularly, as in the reduced models discussed earlier, with adapters the pretrained original transformer $F$ first caches the intermediate activations $h^{k}_{c\in\mathcal{C}}$ for each input in a selected corpus at layer $k$. Then the first $k$ layers are removed from the transformer. During fine-tuning, the cached representations are fed as input to the later $N-k$ layers of the transformer, which consist of the frozen transformer layers plus trainable adapter parameters. Thus, we fine-tune only the additional 6-8\% parameters introduced by the adapters.
% since only the adapter parameters need to be stored, which can be cached and retrieved alongside a base model at runtime. 
We refer to learning adapters on all layers as the {\em full adapter} setting and the layer recycling version as the {\em reduced adapter} setting.

% We explore how precomputed embeddings can be reused within variations of the BERT and T5 transformer architectures. Within the transformer architecture, activations are generated at each transformer layer sequentially before being fed into the next layer in the model. In our within-model approach, we use a \textit{source model} to run over a selected corpus before our experiments, caching the outputted hidden state from a specific intermediate layer for each input locally. During the experiments, a \textit{consumer model} then uses the cached hidden states for fine-tuning and testing. Both the source model and the consuming model have the same architecture.

% For within-model recycling, we experiment with two different setups. The first setup is semi-frozen models, in which earlier layers of BERT models are frozen from fine-tuning. Through this configuration, our source model gathers the embeddings for each input in a selected corpus, caching the intermediate hidden state from the last frozen transformer layer before the later unfrozen layers. For the consumer model, we can then remove the earlier BERT layers that are frozen from fine-tuning and feed the cached hidden states directly into the reduced model with only fine-tunable layers. 

% The second setup is Adapter-based models, in which Adapter modules \citep{houlsby2019parameter} are added to the latter half of transformer layers in frozen transformer models. In this approach, the source model also caches the intermediate hidden states for each input in a selected corpus, collecting the hidden states from the last transformer layer before the layers with Adapters. For the consumer model, we remove the earlier BERT layers that are frozen from fine-tuning before feeding the cached hidden states directly into the reduced model, which includes only the frozen layers that have trainable Adapters attached.


\section{Experimental Setup}

We now present our experiments evaluating whether recycled embeddings can be paired with reduced large language models to maintain accuracy while improving training and inference speed.  We explore the effectiveness of embedding recycling across a variety of different tasks, datasets, and transformer models.

\subsection{Models} 
% Based on the multi-layer bidirectional Transformer \citep{vaswani2017attention},
Our full-size models include the encoder transformers  BERT, SciBERT \citep{beltagy2019scibert}, RoBERTa \citep{liu2019roberta}, and DeBERTa \citep{he2020deberta}. We also experiment with the encoder-decoder T5 model \citep{raffel2019exploring}.
%\chrisc{it might be important to specify that T5 is an encoder-decoder model}
We selected these architectures since they are widely-used pretrained transformers across a variety of tasks in different domains. We experiment with multiple sizes of these models, including distilled \citep{sanh2019distilbert,wang2020minilm, wang2021minilmv2}, base, and large variants, to gauge the effectiveness of recycled embeddings with an increase in the network size.

To investigate the effectiveness of layer recycling, we test several reduced models in which we use caching to reduce 50\% of the layers (e.g., caching layer 12 in RoBERTa-large and layer 6 in BERT-base).\footnote{We note that for the encoder-decoder model T5, we consider caching only the middle layer of the {\em encoder}, which means that the speedups for this model will be smaller than (approximately half of) that of the other models we evaluate.  We also consider 25\% and 75\% reduced models in \autoref{sec:experimental_setup}.}  We compare each reduced model to its fully fine-tuned counterpart across the text classification, NER, and QA tasks. The hardware details and hyperparameters for our models are specified in \autoref{sec:experimental_setup}.

% they serve as the current state of the art \arman{These are not state of the art, I'll rephrase}

% Each model has a different number of transformer layers. RoBERTa-Large has 24 transformer layers, BERT-base and SciBERT have 12 layers, and DistilBERT and MiniLM, have 6 transformer layers each. The encoder and decoder side of T5-base (T5-3b) have 12 (24) layers each. T5 models were originally pretrained on a multi-task mixture of unsupervised and supervised tasks, such as question-answering, sentiment analysis, and natural language inference. RoBERTa and BERT, along with distilled versions of the models, were pretrained on the Masked language modeling (MLM) objective using a large corpus of English data. 

\subsection{Datasets}

For our experiments, we focus on three core NLP tasks: text classification, named-entity recognition (NER), and extractive question-answering (QA). Scientific papers, due to their immutable nature, are an especially appropriate target for embedding recycling, so we focus much of our evaluation on the scientific domain.  For text classification, we selected Chemprot \citep{kringelum2016chemprot}, SciCite \citep{cohan-etal-2019-structural}, and SciERC \citep{luan2018multi}. For NER, we used BC5CDR \citep{li2016biocreative}, JNLPBA \citep{collier2004introduction}, and NCBI-Disease \citep{dougan2014ncbi}. For QA, we chose the TriviaQA \citep{joshi2017triviaqa} and SQuAD \citep{rajpurkar2016squad} datasets. 


==> submissions/TMLR August 2022/3-results.tex <==


\section{Results}
\label{sec:results}

\subsection{Standard Fine-tuning}

%\mike{Hmm, I have mixed feelings about referring to these models as being "able" or "unable" to do things; seems like a strong claim given that we didn't test configurations exhaustively.  Perhaps "did" or "did not".}

%\mike{Need to define "matches", and may need to adjust claims for "matches or outperforms" depending on how we define it.  See Slack discussion: https://allenai.slack.com/archives/C03D8LCAXMG/p1656716209218279}

\input{meta_results_table.tex}

The results for standard fine-tuning of either full or reduced models are shown in \autoref{tab:metatable}.  For the text classification and NER tasks, the reduced BERT-sized and larger models perform similarly to their fine-tuned counterparts on average, and substantially outperform the distilled models.  The reduced distilled models also perform well on those tasks compared to the distilled originals, on average, although there is more variance across models and tasks compared to BERT-sized models. We validate our fully fine-tuned baselines by comparing our results with prior work \citep{beltagy2019scibert}, finding that our scores land within 1.33\% on average and typically score above the previous baselines.
%across the tasks and models For text classification, even with 50\% of the layers frozen, RoBERTa-Large, MiniLM L6-H384, and DistilBERT were able to match or outperform their respective fully fine-tuned configurations. %However, freezing MiniLM L6-H768 layers did not seem to be at par with full fine-tuning.

%For NER, reduced RoBERTa-Large, SciBERT, MiniLM L6-H768, and DistilBERT were generally on par with their respective fully fine-tuned configurations. However, reduced MiniLM L6-H384 did not seem to match the full fine-tuning.

For QA tasks, we found that fully fine-tuning works somewhat better than reduced configurations across all the explored models (\autoref{tab:metatable}). Generally, reduced configurations typically lag by 1 to 2 points in F-1 score.  One possible hypothesis is that the QA datasets are generally much larger than the datasets we used for other tasks (100k-150k examples vs 4k-20k examples for text classification and NER); however, in additional experiments we found that subsampling the QA training sets to 5\% of their original size only increased the gap, suggesting that dataset size does not explain the failure of reduced models on this task.  %As shown in \autoref{sec:experimental_setup}, reducing the model by only 25\% is substantially more effective for QA (average F1 drops by 0.2-0.5 points), which suggests that training layers some of the earlier layers is important for the model to achieve its best performance on the QA datasets, and that future work may consider task-specific choices for which layer to recycle.
We also validate our fully fine-tuned baselines for QA tasks by comparing our results with prior work \citep{yasunaga2022linkbert}, finding that our scores land within 0.42\% on average.
%Despite the accuracy drop, our QA results compare favorably with previous work.  The QA-specific decomposition techniques in \citep{cao2020deformer} 

Additionally, we explored using lightweight multi-layer perceptrons (MLPs) as classifier heads, given their success in previous work. While \cite{du2020general} paired multi-task encoders with 2-layer MLPs, we paired frozen pretrained transformer models with 2-layer MLPs and found that they underperformed trainable layers dramatically, by 26\% on average across the text classification and NER tasks. %Furthermore, we found that using a 2-layer MLP instead of a standard linear classifier head in our embedding recycling approach did not meaningfully improve F1-score across text classification, NER, and QA tasks. 
%\jon{Double check phrasing of this paragraph} 
%\dd{I might cut the furthermore sentence here, since it's a somewhat different point (about a design decision within our approach, rather than a comparison vs. Du et al's approach).  You could mention this choice of linear vs. MLP in Sec 4.1 or maybe appendix.}

\subsection{Adapters}

\input{adapters_results.tex}

Our results for reduced adapter models are shown in \autoref{tab:adapters}.  We see that in general, for all the models except for T5-Large, the adapter-based approaches are superior to standard fine-tuning on our tasks.  Further, layer recycling remains effective with adapters.  Compared to the full adapter baseline, the reduced adapters for RoBERTa-Large, BERT, and SciBERT models only show a 0.15-0.17\% reduction in accuracy. Additionally, compared to the fully fine-tuned baseline, these reduced adapters models have a 0.19-0.23\% reduction in accuracy. 
%\jon{Should we compare to fully finetuned like the abstract or full adapter baselines, as it is now?} \dd{Good question, I'd suggest adding an additional sentence comparing against full fine-tuned; fortunately it makes almost no difference since the numbers are very similar in the two cases?} 
Likewise, in contrast to the full fine-tuning results above, QA accuracy for the top-performing DeBERTa adapter model remains unchanged on average after layer recycling, with the reduced adapter model performing better on one QA task and worse on the other.\footnote{We omit experiments with distilled models, as we found adapters to be ineffective on those models even without embedding recycling, scoring 19.4\% worse on average than full fine-tuning for text classification and NER.} 
%\arman{Consider moving the last sentence to footnote.}

\subsection{Efficiency Analysis}
\label{sec:performance_analysis}

\begin{table}[ht]
\footnotesize
\centering
\small
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4.3pt}
\begin{tabular}{ccccccc} 
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{1}{c}{\multirow{3}{*}{\textbf{Baseline} (NR)}} & \multicolumn{2}{c}{\textbf{Inference Time} (ms/batch)} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Speedup}}} & \multicolumn{1}{c}{\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Avg. F1} \\ \textbf{Loss} using \\ \textbf{Recycling}\end{tabular}}}  \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{2}{c}{\textbf{\textbf{Recycling}}} & \multicolumn{2}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{FP32 Cache} & \multicolumn{1}{c}{FP16 Cache} & \multicolumn{1}{c}{NR vs FP32} & \multicolumn{1}{c}{NR vs FP16} \\
\midrule
\multicolumn{6}{c}{NVIDIA A10G} \\
$\text{MiniLM}_{384}$ & 183 $\pm$ 1 & 154 $\pm$ 22 & 123  $\pm$ 2 & +21\% & +67\% & -0.2 \\
$\text{MiniLM}_{768}$ & 325 $\pm$ 1 & 201 $\pm$ 11 & 195  $\pm$ 4 & +56\% & +66\% & -0.4 \\
$\text{BERT}_{\textsc{Base}}$ & 647 $\pm$ 1 & 351 $\pm$ 1 & 343  $\pm$ 5 & +84\% & +88\% & -0.3 \\
$\text{BERT}_{\textsc{Large}}$ & 1943 $\pm$ 1 & 1066 $\pm$ 12 & 1004  $\pm$ 4 & +86\% & +93\% & -0.2 \\
$\text{DeBERTa}_{\textsc{XLarge}}$ & 1914 $\pm$ 2 & 1010 $\pm$ 10 & 985 $\pm$ 8 & +89\% & +94\% & -0.1 \\
\midrule
\multicolumn{6}{c}{NVIDIA A6000} \\
$\text{MiniLM}_{384}$ & 123 $\pm$ 1 & 105 $\pm$ 5 & 100  $\pm$ 2 & +18\% & +23\% & -0.2 \\
$\text{MiniLM}_{768}$ & 208 $\pm$ 1 & 161 $\pm$ 8 & 150  $\pm$ 4 & +29\% & +38\% & -0.4 \\
$\text{BERT}_{\textsc{Base}}$ & 416 $\pm$ 1 & 269 $\pm$ 6 & 245  $\pm$ 2 & +55\% & +59\% & -0.3 \\
$\text{BERT}_{\textsc{Large}}$ & 1235 $\pm$ 1 & 662 $\pm$ 10 & 643  $\pm$ 10 & +86\% & +92\% & -0.2 \\
$\text{DeBERTa}_{\textsc{XLarge}}$ & 1430 $\pm$ 2 & 777 $\pm$ 6 & 758 $\pm$ 4 & +84\% & +89\% & -0.1 \\
\bottomrule
\end{tabular}
\caption{
Average \textbf{inference} runtime comparison (in ms per batch, $\pm$ stdev over 7 runs) between vanilla encoders and models that cache embeddings on disk. 
We assume the cache is precomputed (see \autoref{sec:performance_analysis}). 
For all runs, cache the middle layer of the encoder; thus, maximum speedup is 100\%.
Overall, the larger the model, the higher the speedup from re-using representations. 
Further, accelerators with fewer execution units (A10G) benefit more from recycling embeddings. 
Finally, using half precision for embedding caching improves speed up across the board, while halving storage size. We also found that half-precision has a negligible effect on F1-scores at inference if you originally train the models using full-precision. In the rightmost column, we included the average F1 loss from using embedding recycling across our tasks.}
\label{tab:performance}
\end{table}


\begin{table}
\footnotesize
\centering
\small
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4.3pt}
\begin{tabular}{cccccccc} 
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\textbf{Training} (ms/batch, amortized over \textbf{ 6 epochs})} & \multicolumn{3}{c}{\textbf{Speedup}} \\
 & \begin{tabular}[c]{@{}c@{}}\textbf{No}\\\textbf{Recycling} (NR)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Model}\\\textbf{Frozen} (F)\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}}\textbf{Saving} \textplus \\\textbf{Recycling} (SR)\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}c@{}}\textbf{Only} \\\textbf{Recycling} (R)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{NR} vs\\ \textbf{SR}\end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{F} vs\\ \textbf{SR}\end{tabular} &  \begin{tabular}[c]{@{}c@{}}\textbf{NR} vs\\ \textbf{R}\end{tabular} \\
\midrule
\multicolumn{8}{c}{NVIDIA A10G} \\
$\text{MiniLM}_{384}$ & 51 $\pm$ 1 & 30 $\pm$ 1 & 32 $\pm$ 6 & 25 $\pm$ 4 & +59\% & -7\% & +104\% \\
$\text{MiniLM}_{768}$ & 90 $\pm$ 4 & ~56 $\pm$ 1 & 50 $\pm$ 4 & 45 $\pm$ 3 & +80\% & +12\% & +100\% \\
$\text{BERT}_{\textsc{Base}}$ & 173 $\pm$ 2 & 112 $\pm$ 1 & 90 $\pm$ 4 & 87 $\pm$ 3 & +92\% & +24\% & +99\% \\
$\text{BERT}_{\textsc{Large}}$ & 347 $\pm$ 1 & 246 $\pm$ 1 & 181 $\pm$ 2 & 176 $\pm$ 2 & +92\% & +36\% & +97\% \\
$\text{DeBERTa}_{\textsc{XLarge}}$ & 380 $\pm$ 2 & 286 $\pm$ 1 & 199 $\pm$ 1 & 194 $\pm$ 1 & +91\% & +44\% & +96\% \\
\midrule
\multicolumn{8}{c}{NVIDIA A6000} \\
$\text{MiniLM}_{384}$ & 41 $\pm$ 1 & 24 $\pm$ 1 & 26 $\pm$ 5 & 22 $\pm$ 3 & +55\% & -8\% & +81\% \\
$\text{MiniLM}_{768}$ & 61 $\pm$ 1 & 38 $\pm$ 1 & 40 $\pm$ 5 & 34 $\pm$ 3 & +52\% & -5\% & +82\% \\
$\text{BERT}_{\textsc{Base}}$ & 117 $\pm$ 1 & 78 $\pm$ 1 & 60 $\pm$ 3 & 58 $\pm$ 2 & +94\% & +30\% & +102\% \\
$\text{BERT}_{\textsc{Large}}$ & 326 $\pm$ 2 & 212 $\pm$~1 & 167 $\pm$ 2 & 161 $\pm$ 1 & +96\% & +26\% & +103\% \\
$\text{DeBERTa}_{\textsc{XLarge}}$ & 359 $\pm$ 2 & 250 $\pm$~1 & 184 $\pm$ 1 & 178 $\pm$ 1 & +95\% & +35\% & +102\% \\
\bottomrule
\end{tabular}
\caption{
Average \textbf{training} runtime comparison (in ms per batch, $\pm$ stdev over 7 runs) between vanilla encoders and models that cache embeddings on disk. 
For all runs, we cache the middle layer of the encoder; thus, theoretical speedup is 100\%. 
Time per batch is amortized over 6 epochs ($2,000$ steps), the lowest number to convergence over all datasets (c.r.f. Table~\ref{tab:training_times}). 
We present results in four settings: no recycling (NR), freezing \textonehalf~of the layers during training (F), 1 training epoch during which embeddings are saved to disk followed by 5 epochs where recycling is enabled (SR), and 6 epochs where embeddings are already saved (R).
Overall, we found that embedding recycling speeds up training even when embeddings need to be cached to disk during the first pass.
Compared to freezing, saving and recycling improves training time for all but  MiniLM models (F vs SR).
}
\label{tab:performance_training}
\end{table}

To estimate the real-world benefit of recycling embeddings for different tasks, we provide a minimal PyTorch implementation of embedding recycling.\footnote{Code and documentation available in supplementary material.} 
This implementation and the following results correspond to both the standard layer recycling approach and the adapter-based layer recycling approach since they follow parallel processes for gradient descent during training and computations during inference, despite the additional 6-8\% of parameters added by the trainable adapters. To show that training times do not differ substantially, we also measured the training time the transformer models take to converge to their optimal weights. We found both approaches take approximately the same training time to complete training (\autoref{tab:training_times}).

We evaluated the impact of recycling embeddings on four different architectures and two different hardware platforms. 
For models, we considered two efficient transformer models (Two 6-layer MiniLMv2 \citep{wang2020minilm,wang2021minilmv2} models with embeddings of size 384 and 768), a base model ($\text{BERT}_{\textsc{Base}}$ uncased, 12 layers and 768 dimensional embeddings), and a large model ($\text{BERT}_{\textsc{Large}}$ uncased) with 24 layers and embeddings of size 1024. 
Intuitively, we expect larger models with more layers to benefit more from embedding recycling. 
For platforms, we ran our proof-of-concept implementation on an AWS cloud instance\footnote{ \texttt{g5.2xlarge} instance with 8 cores and 32 GB of RAM.} equipped with an NVIDIA A10G accelerator, and on a NVIDIA A6000 within an on-premise server\footnote{Intel-based system with 128 cores and 512 GB of RAM.}. 
The former contains fewer execution units (72 vs 84), fewer tensor cores (288 vs 336), slower memory (600 vs 768 GB/s), and slower boost clock (1800 MHz vs 1695 MHz). However, it is much more efficient, being rated at 150W (compare with A6000's 300W power target). 
Therefore, the NVIDIA A10G accelerator presents a more realistic platform for embedding recycling, since it is more suitable for cost-efficient large-scale model deployments.
Both machines are equipped with PCIe NVMe drives, which we use to cache embeddings to recycle. 

~\autoref{tab:performance} shows the results of caching embeddings to recycle on disk.
% Because inference speed is similar across all tasks, 
Because inference time varies across tasks depending on dataset properties, such as length of sequences and number of samples, we control our experiments by simulating a sequence classification task on \textsc{Qasper} \citep{dasigi2021qasper}, which includes the full-text of over a thousand academic manuscripts.\footnote{Because the bulk of computation for a transformer model is done in its encoder and not in the task-specific heads, inference time is similar regardless of whether the model is used for sequence classification, tagging, or question answering.}
Further, we run all models with a fixed batch size of 128 and maximum sequence length of 512; 
for all models, we reduce exactly half of their layers by recycling, which results in a maximum theoretical speed-up of 100\%.  A run over the corpus consists of 335 batches, and we average results over seven runs.
Overall, we found that in practice all models benefit from embedding recycling, achieving an average speedup ranging from 18 to 86\%. 
Unsurprisingly, larger models benefit more from recycling than smaller ones; this is due to the fact that loading embeddings cached on disk adds a small latency penalty to a model run, which is more noticeable in the case of smaller models. 
For example, we achieve an 84\% speedup when running $\text{BERT}_{\textsc{Base}}$ with embedding recycling on an A10G GPU, which is roughly equivalent to the latency of a $\textsc{MiniLM}_{768}$ model without recycling (351 vs 325 ms per batch on average);
this result would us allow to run more accurate models while maintaining the efficiency of shallower architectures. 

We note that in our inference-time speedup measurements, we assume that the cache is already precomputed.  This corresponds to our target setting in which new tasks and models are executed over the same text that has been processed previously.  Because the cost to write the cache to disk is approximately equal to a single inference pass over the corpus, if we perform $t$ total inference passes for different models/tasks given the same precomputed cache, the total amortized speedup will be approximately $\frac{t}{t+1}$ of the values we report in \autoref{tab:performance}. Thus, as the number of inference passes to be run increases, the total amoritized speedup including the cost to write the cache will approach the values reported in the table.

\autoref{tab:performance} also includes results when storing embeddings using half precision (that is, cache embeddings in FP16 rather FP32). When using half precision, we observed improvements for all models and hardware, ranging from $+8\%$ to $+46\%$. 
Storing cached embeddings in FP16 has virtually no impact on performance, as it changes predicted scores by typically $10^{-3}-10^{-5}$ across all tasks evaluated in this work.


We also note that less capable hardware benefits more from caching embeddings. 
For example, $\text{BERT}_{\textsc{Base}}$ achieves a speedup of $84\%$ on an A10G GPU, while on A6000, the speedup is a more modest $55\%$. 
This is an expected result: fewer and slower execution cores/accelerator memory impact overall model latency.
Further, we note that, despite the smaller relative gains, the more powerful GPU is always faster in absolute terms compared with the less capable one.

It is important to note that these gaps from  maximum achievable speedup are only observed when performing \textit{inference}; 
for \textit{training}, we observe almost perfect speed-up for all models and hardware configurations  barring MiniLM models on the machine equipped with a A6000 GPU (``NR vs R'' column in \autoref{tab:performance_training}).  
For example, $\text{BERT}_{\textsc{Base}}$ requires $17.38 \pm 1.32\text{ ms/batch}$\footnote{When training, we use a batch size of 16} without recycling, compared to $8.67 \pm 2.18\text{ ms/batch}$ when recycling.
Even when considering the additional time to cache embeddings to disk during the first pass, embedding recycling still achieves close to optimum speedup on all models except MiniLMs, where its gains hover between 52\% and 82\% (``NR vs SR'' column in \autoref{tab:performance_training}).
When training for just 6 epochs (or roughly $2,000$ steps), recycling embeddings is faster than simply freezing half of the parameters for all models but MiniLM (``F vs SR'' column in \autoref{tab:performance_training}); this is due to the relatively higher cost of caching layers to disk in case of smaller models.
In these cases, we empirically found that recycling achieves faster training time than freezing after 12 epochs or $4,000$ training steps; 
since smaller models typically require more epochs to converge, we conclude that recycling is generally preferable to partially freezing a model during training.

We also benchmarked the storage requirements of recycling embeddings. 
For a sequence of 512 tokens and a hidden model dimension of 768, caching embeddings requires 1.6 MB. 
In practical terms, this translates to 15.5 MB per paper in \textsc{Qasper} (papers are, on average 4,884 WordPiece tokens in length).
%We note that the storage requirement could be optimized using half-precision floating points and compression techniques, which we did not investigate in this work. 
Besides the storage needs, NVMe disks, while fast, introduce additional latency compared to RAM. 
For example, $\text{BERT}_{\textsc{Base}}$ achieves an average latency of $351 \pm 1 \text{ ms/batch}$ when caching on disk ($84\%$ speedup), compared to just $334 \pm 1 \text{ ms/batch}$ when using memory ($94\%$ speedup). 
To reduce the impact of this latency penalty, our implementation supports \textit{pre-fetching} of future embeddings: when processing a sequence of inputs, such as sentences in a manuscript, it loads embeddings for tokens ahead of the sequence inference is currently being run on.
This optimization reduces the time accelerators wait for data to be available for inference; 
for example, in the case of $\text{BERT}_{\textsc{Base}}$ on A10G, disabling pre-fetching raised inference inference time to $374 \pm 1 \text{ ms/batch}$ (vs $351 \pm 1 \text{ ms/batch}$ with pre-fetching). 
Therefore in this section, all results are reported with prefetching enabled.

% In contrast to latency, throughput requirements are less severe: we measured peak read speed of $384\text{ MB/s}$ when loading recycled embedding from disk, suggesting that, if streamed over the network, a $5\text{ Gbps}$ connection would be sufficient.


==> submissions/TMLR August 2022/4-discussions.tex <==


\section{Discussion}



%For text classification tasks, we found that both frozen RoBERTa and SciBERT with adapters on the latter half of their transformer layers outperform their respective fully fine-tuned versions substantially on SciERC-Rel and slightly on ChemProt, but underperform on SciCite.  The differences between the adapter-augmented and fully-finetuned models are smaller for the NER datasets, and have approximately equal performance on average.

\subsection{Cross-model Embedding Reuse}

\input{AppendixTables/CrossModelExperiments}

The experiments in \autoref{sec:results} focus on caching activations from a pretrained model and then re-using those for fine-tuning and inference with the same model.  An alternative potential use-case of ER involves caching activations from a more expensive, larger model once and re-using those downstream within a cheaper model multiple times.  Here, the goal is not to improve efficiency of the downstream model, but instead to improve its accuracy by introducing the helpful contextual embedding signal from the larger model.  However, as we will show, a straightforward implementation of this strategy did not offer improvements in our experiments.

We experiment with reusing precomputed embeddings from one source model $F$ in a consumer model $F'$ that has a different transformer architecture but the same tokenization vocabulary. During the caching step for the source model, the activations of the \emph{final} transformer layer $h^{N}_{c\in\mathcal{C}}$ are stored for each input $c$ of the selected corpus $C$. During the fine-tuning phase of the consumer model $F'$, these stored activations are transformed through a learned 2-layer MLP and added to the input embeddings of $F'$.
%combined with the input embeddings of the consumer model before being fed into the consumer model's encoder.
%The objective of this setup is to increase richness of the representations in the compact consumer models $F'$ through the addition of activations from a larger source model $F$.

%
%\subsection{Dataset Size}
%
%For the within-model recycling experiments, we found that reduced and adapter-based configurations of transformer models were able to match or outperform fully fine-tuned transformer models on text classification and NER tasks. For QA tasks, however, these configurations were not able to match fully fine-tuned model performances. From further experimentation, we attribute the lower performances on QA tasks to the different dataset sizes.
%\aps{I don't understand the comment in the last sentence, probably frame it in a way such that we can say our approach works better for small datasets/lower resource settings?}
%\jon{I should probably remove this comment about QA dataset size being the issue. I can also mention the positive results for the T5 experiment?}
%
%The text classification and NER datasets ranged in overall size from ~4,000-20,000 datapoints (\autoref{tab:datasets}). The QA datasets, however, ranged in overall size from ~100,000-150,000 data points, making them an order of magnitude larger than the other datasets. We explored whether the larger dataset sizes led to reduced performance for within-model recycling by sampling ~7,000 datapoints from the QA datasets rather than using the entire datasets. We found that \jon{Add info on these results once completed} 

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[t]
% \begin{tabular}{lll}
% \toprule
% \textbf{Task}                                                                   & \textbf{Dataset} & \textbf{\begin{tabular}[c]{@{}l@{}}Number of\\ Examples\end{tabular}} \\ \midrule
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Text \\
% Classification\end{tabular}} & ChemProt         & 10,065                                                             \\ 
%                                                                                 & SciCite          & 10,097                                                             \\
%                                                                                 & SciERC-Rel       & 4,648                                                              \\ \cdashline{0-2}
% \multirow{3}{*}{NER}                                                            & bc5cdr           & 12,030                                                             \\
%                                                                                 & JNLPBA           & 22,402                                                             \\
%                                                                                 & NCBI-disease     & 7,287                                                              \\ \cdashline{0-2}
% \multirow{2}{*}{QA}                                                             & TriviaQA         & 141,324                                                            \\
%                                                                                 & SQuAD            & 98,169 \\
%                                                                                 \bottomrule
% \end{tabular}
% \caption{Sizes of datasets for text classification, NER, and QA tasks}
% \label{tab:datasets}
% \end{table}

Using our text classification tasks, we tried two frameworks for pairing large language model embeddings with compact models. In our first framework, we use a frozen RoBERTa model as our source model and a MiniLM-6L-H768 model as our consumer model. In our second framework, we use a frozen BERT-base model as our source model and a DistilBERT model as our consumer model.
%ReLU
We use a ReLU activation in the 2-layer MLP.  In our testing, we also explored using a single linear layer rather than an MLP but found an MLP achieved better performance on the development sets for the text classification tasks.
The results of our experiments are shown in \autoref{tab:crossmodel}.  Overall, the larger model's contextual representations do not improve the smaller model's accuracy; in fact adding them decreases the average F1 score by 0.3-0.9 points.  %In future work, we hope to explore different approaches for cross-model recycling.

\subsection{GLUE Results}

\input{AppendixTables/NLI_Results}

For our best-performing model DeBERTa v2 XL, we also provide further experiments on datasets from the GLUE benchmark \citep{wang2018glue}, to allow easier comparison against speedup techniques from previous work.  In this revision we present preliminary results on the CoLA, SST-2, MRPC, STS-B, MNLI, and QNLI tasks from GLUE. For our experiments, we tried both our standard reduced models and our reduced adapter models. We found that embedding recycling was successful across the GLUE tasks, with a small loss in F1 scores in return for a significant increase in both training and inference time as outlined in \autoref{tab:performance} and \autoref{tab:performance_training}.  We note that due to the high computational cost of these experiments, we take existing hyperparameter settings from previous work that worked well for the full models, and also use these for reduced models.  Further hyperparameter optimization of the reduced models might improve performance.

%\subsection{Early Exiting}

%\input{AppendixTables/Early_Exiting_Results}

%We also explored whether embedding recycling can be used successfully alongside other efficiency techniques. Specifically, we tested embedding recycling with the DeeBERT early exiting strategies \citep{xin2020deebert}, which include ``off-ramps'' that allow a model to not compute later layers of a model when the model is already confident of the classification from earlier layers. For our combined early exiting and embedding recycling experiments, we tested two of our best performing models, RoBERTa-Large and DeBERTa V2 XL, across our text classification, NER, and QA tasks. %The original DeeBERT experiments only explored the GLUE classification tasks so we wanted to see if early exiting strategies could succeed on other tasks.

%We find that with a small loss in F1, early exiting can be successfully paired alongside embedding recycling for text classification tasks using RoBERTa-Large and DeBERTa V2 XL (\autoref{tab:early_exiting}). We found that with a 0.5-1.5 point loss in F1, we can gain up to 38\% inference time decrease for RoBERTa-Large and 22\% inference time decrease for DeBERTa V2 XL. When combined with the inference time gains made from embedding recycling, this leads to a \textasciitilde $4x$ speedup in inference.

%For NER tasks, we also found that a 0.1-1.5 point loss in F1 can yield up to a 39\% inference time decrease for RoBERTa-Large. For DeBERTa V2 XL, however, we found the tradeoff to be less favorable, with a 3-5 point loss in F1 for a 12-31\% decrease in inference time. Additionally, early exiting paired with embedding recycling seemed generally less effective on QA tasks; a 2-3 points loss in F1 corresponded with roughly a 13-15\% decrease in inference time for both RoBERTa-Large and DeBERTa V2 XL. \jon{Checkout writing of these two paragraphs}

\subsection{Directions for Future Work}

Our experiments raise several questions that could be answered in future studies, and embedding recycling contains a much larger space of potential techniques than those we investigate here.  Future work could proceed along various lines, including:
\begin{itemize}
    \item Our layer recycling strategy is a straightforward ER approach, but previous work has suggested that weighted pooling across layers can perform better %in probing tasks
    compared to any single layer in many cases \citep{liu-etal-2019-linguistic,du2020general}.  Recycling pooled activations may offer improved results.  What is the best way to capture and store the syntactic and semantic knowledge encoded in the activations of a model for later recycling?
    \item Our experiments show that the right recycling approach may be task-specific and model-specific.  For example, with standard fine-tuning as shown in \autoref{tab:roberta}, caching layer 12 in RoBERTa-large is most effective for NER and text classification, whereas it is not effective for QA (but layer 6 performs much better).  Which embeddings to retrieve and recycle for a task, and the right architecture (e.g. number of layers) to use when consuming the recycled embeddings, represents a large decision space.  Methods that can help practitioners automatically choose among public or private shared embedding sets and associated model designs, given their task and objectives for accuracy and computational cost, may be important to make ER an effective practical tool.
    \item We present results with encoder-only and encoder-decoder models, on classification tasks.  Determining the approach is effective for generative tasks and autoregressive models is an important question for future work.
    \item Other than recycling, a variety of other inference-speedup techniques exist for large neural models.  While we show that ER can be effective when coupled with distillation, whether other techniques like quantization and early exiting remain effective in combination with ER is an open question. %One  straightforward and potentially promising direction would be to combine the "late start" of layer recycling ER with early exit techniques \citep{xin2020deebert}. 
    \item We focus on the setting where the exact same text, at the length of a full document, is being reused for multiple tasks.  In practice, we may often perform a task on text that is {\em similar} to but not exactly the same as one for which we have cached embeddings (e.g., a Wikipedia page that has been revised).  Further, even a completely new document will have similarities and overlapped spans with previously processed ones.  Studying ER in these settings, e.g. through a combination of layer recycling and the SkipBERT approach which can apply to unseen passages via cached n-grams \citep{wang2022skipbert}, is an area of future work.
    \item Finally, our techniques for cross-model embedding reuse were not effective in our experiments.  However, using rich contextualized embeddings from a large model to help power many smaller downstream task models is an important setting for ER, since it provides a powerful way to amortize the expense of running a large model. Developing and evaluating new approaches for this setting is an important item for future work.
\end{itemize}



==> submissions/TMLR August 2022/5-conclusion.tex <==


\section{Conclusion}

We have presented embedding recycling, a general technique for reusing previous activations of neural language models to improve the efficiency of future training and inference.  We show how a simple technique of caching a layer of activations in a pretrained model is effective.  We validate our approach in experiments across eight tasks and seven model architectures.  We find that recycling typically has small or no impacts to accuracy on average, but does yield substantial throughput increases demonstrated through a careful efficiency analysis.  We also discuss several open challenges for future work.



==> submissions/TMLR August 2022/CrossModelExperiments.tex <==


\begin{table*}[htp]
\centering
\small
\begin{tabular}{llrrrr}
\toprule
                                                         & \textbf{}                                     & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}RoBERTa-Large\\ + MiniLM L6-H768\end{tabular}}} & \multicolumn{1}{l}{\textbf{MiniLM L6-H768}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}BERT + \\ DistilBERT\end{tabular}}} & \multicolumn{1}{l}{\textbf{DistilBERT}} \\ \midrule
\textbf{Chemprot}                                        & Micro F-1                                     & 78.9 (0.3)                                                                                            & \multicolumn{1}{r}{{79.3 (0.3)}}    & 77.8 (0.4)                                                                                & {79.1 (0.5)}                     \\
\textbf{}                                                & Macro F-1                                     & 52.2 (0.2)                                                                                            & \multicolumn{1}{r}{{52.6 (0.4)}}    & 51.2 (0.5)                                                                                & {52.6 (0.3)}                     \\
\textbf{SciCite}                                         & Micro F-1                                     & 85.2 (0.3)                                                                                            & \multicolumn{1}{r}{{86.0 (0.2)}}    & {85.7 (0.1)}                                                                       & 85.5 (0.1)                              \\
\textbf{}                                                & Macro F-1                                     & 83.8 (0.3)                                                                                            & \multicolumn{1}{r}{{84.6 (0.2)}}    & {84.2 (0.1)}                                                                       & 84.0 (0.1)                              \\
\textbf{SciERC-Rel}                                      & Micro F-1                                     & 85.1 (0.4)                                                                                            & \multicolumn{1}{r}{{86.3 (0.2)}}    & {83.8 (0.2)}                                                                       & 83.5 (0.4)                              \\
                                                         & Macro F-1                                     & 76.2 (0.8)                                                                                            & \multicolumn{1}{r}{78.2 (0.6)}    & {73.6 (0.6)}                                                                       & 72.9 (0.7)                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Text Classification\\ Average Score\end{tabular}}} & 76.9                                                                                                  & \multicolumn{1}{r}{\textbf{77.8}}          & 76.0                                                                                      & \textbf{76.3}  \\ \bottomrule                        
\end{tabular}
\caption{Cross-Model Recycling Results for RoBERTa+MiniLM-L6H768 and BERT+DistilBERT configurations. \textbf{Bold} indicates the best average score between the cross-model recycling and fully finetuned versions of each model. Each score represents the average score of 10 runs, with the standard errors for each score in parentheses.}
\label{tab:crossmodel}
\end{table*}

==> submissions/TMLR August 2022/DeBERTa_v2_XL.tex <==


\begin{table*}[htp]
\centering
\small
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{llrrrrrr}
\toprule
                                                          &                                              & \multicolumn{1}{l}{}                                                                          & \multicolumn{1}{l}{}                                                                           & \multicolumn{4}{c}{\textbf{DeBERTaV2 XL}}                                                                                                                                                                                                                                                                                                                                                    \\ \midrule
                                                          & \textbf{}                                    & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Reduced +\\ Half Adpt\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Full \\ Adapters\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}6 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}12 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}18 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Fully \\ Finetuned\end{tabular}}} \\ \midrule
\textbf{ChemProt}                                         & Micro F-1                                    & \textbf{87.2 (0.1)}                                                                           & 86.5 (0.2)                                                                                     & \textbf{87.2 (0.2)}                                                                            & 86.8 (0.4)                                                                                      & 86.4 (0.2)                                                                                      & 86.7 (0.9)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 56.7 (0.5)                                                                                    & 55.6 (0.6)                                                                                     & \textbf{59.6 (0.2)}                                                                            & 59.5 (0.5)                                                                                      & 59.2 (0.3)                                                                                      & 59.0 (1.1)                                                                              \\
\textbf{SciCite}                                          & Micro F-1                                    & 85.8 (0.4)                                                                                    & \textbf{86.4 (0.4)}                                                                            & 86.0 (0.1)                                                                                     & 86.3 (0.2)                                                                                      & 86.2 (0.3)                                                                                      & 85.9 (0.2)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 84.6 (0.4)                                                                                    & 85.0 (0.5)                                                                                     & 84.6 (0.1)                                                                                     & \textbf{85.2 (0.1)}                                                                             & 85.0 (0.3)                                                                                      & 84.4 (0.2)                                                                              \\
\textbf{SciERC-Rel}                                       & Micro F-1                                    & \textbf{88.6 (0.5)}                                                                           & 88.0 (0.4)                                                                                     & 88.3 (0.2)                                                                                     & 87.5 (0.1)                                                                                      & 86.6 (0.3)                                                                                      & 88.0 (0.4)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & \textbf{82.9 (0.8)}                                                                           & 82.1 (0.8)                                                                                     & 80.5 (0.5)                                                                                     & 79.9 (0.3)                                                                                      & 78.0 (0.4)                                                                                      & 80.2 (0.5)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Text Classification\\ Average Score\end{tabular}}} & \textbf{81.0}                                                                                & 80.6                                                                                         & \textbf{81.0}                                                                                 & 80.9                                                                                          & 80.2                                                                                           & 80.7                                                                                   \\ \midrule
\textbf{bc5cdr}                                           & Micro F-1                                    & 97.6 (0.0)                                                                                    & 97.7 (0.0)                                                                                     & 97.4 (0.3)                                                                                     & 97.7 (0.0)                                                                                      & 97.6 (0.0)                                                                                      & \textbf{97.9 (0.0)}                                                                     \\
\textbf{}                                                 & Macro F-1                                    & 90.7 (0.1)                                                                                    & 91.1 (0.1)                                                                                     & 89.5 (1.4)                                                                                     & 91.3 (0.0)                                                                                      & 90.9 (0.0)                                                                                      & \textbf{91.8 (0.1)}                                                                     \\
\textbf{JNLPBA}                                           & Micro F-1                                    & 93.6 (0.0)                                                                                    & 93.4 (0.0)                                                                                     & \textbf{93.7 (0.1)}                                                                            & \textbf{93.7 (0.0)}                                                                             & 93.6 (0.0)                                                                                      & \textbf{93.7 (0.0)}                                                                     \\
\textbf{}                                                 & Macro F-1                                    & \textbf{79.3 (0.1)}                                                                           & 79.0 (0.1)                                                                                     & 78.5 (0.3)                                                                                     & 78.5 (0.2)                                                                                      & 77.8 (0.1)                                                                                      & 78.2 (0.1)                                                                              \\
\textbf{NCBI-disease}                                     & Micro F-1                                    & 98.3 (0.0)                                                                                    & 98.4 (0.0)                                                                                     & \textbf{98.6 (0.0)}                                                                            & \textbf{98.6 (0.0)}                                                                             & 98.5 (0.0)                                                                                      & \textbf{98.6 (0.0)}                                                                     \\
\textbf{}                                                 & Macro F-1                                    & 93.3 (0.1)                                                                                    & \textbf{93.5 (0.2)}                                                                            & 93.1 (0.1)                                                                                     & 93.3 (0.1)                                                                                      & 92.8 (0.1)                                                                                      & 93.4 (0.1)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}NER Average \\ Score\end{tabular}}}                & 92.1                                                                                 & 92.2                                                                                           & 91.8                                                                                           & 92.2                                                                                            & 91.9                                                                                            & \textbf{92.3}                                                                           \\ \midrule
\textbf{TriviaQA}                                         & Micro F-1                                    & 78.6 (0.2)                                                                                    & \textbf{79.1 (0.2)}                                                                            & 77.9 (0.2)                                                                                     & 77.4 (0.2)                                                                                      & 77.0 (0.2)                                                                                      & 78.5 (0.1)                                                                              \\ 
\textbf{}                                                 & Macro F-1                                    & 81.6 (0.1)                                                                          & \textbf{82.3 (0.2)}                                                                            & 81.2 (0.1)                                                                                     & 80.6 (0.1)                                                                                      & 80.1 (0.2)                                                                                      & 81.8 (0.1)                                                                              \\ 
\textbf{SQuAD}                                            & Micro F-1                                    & 88.6 (0.0)                                                                                    & 87.2 (0.1)                                                                                     & 88.6 (0.1)                                                                                     & \textbf{88.7 (0.0)}                                                                             & 87.1 (0.0)                                                                                      & 88.5 (0.1)                                                                              \\
                                                          & Macro F-1                                    & \textbf{94.7 (0.0)}                                                                           & 93.9 (0.0)                                                                                     & 94.6 (0.0)                                                                                     & 94.5 (0.0)                                                                                      & 93.5 (0.0)                                                                                      & 94.6 (0.0)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}QA Average\\ Score\end{tabular}}}                  & \textbf{85.9}                                                                                 & 85.6                                                                                           & 85.6                                                                                           & 85.3                                                                                            & 84.4                                                                                            & 85.8  \\ \bottomrule                                                                                 
\end{tabular}
\caption{DeBERTaV2-XL Results for Reduced Models. \textbf{Bold} indicates the best average score between the standard reduced, adapter-based reduced, and fully fine-tuned versions of each model. \textbf{Reduced + Half Adpt} indicates adapters on the transformer layers of a fully frozen reduced model, where the earlier half of transformer layers were removed and their activations cached. \textbf{Full Adapters} indicates adapters on all transformer layers of a fully frozen model. Each score represents the average score of 5 runs, with the standard errors for each score in parentheses.}
\label{tab:deberta}
\end{table*}

==> submissions/TMLR August 2022/DistilBERT_Semifrozen.tex <==


\begin{table*}[ht]
\centering
\begin{tabular}{llrrrr}
\toprule
                                                       &                                                       & \multicolumn{4}{c}{\textbf{DistilBERT}}                                                                                                                                                                                                                                                                                                                                                        \\ \midrule
                                                       & \textbf{}                                  & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}2 Layers \\ Reduced\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}3 Layers \\ Reduced\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}4 Layers \\ Reduced\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Fully \\ Fine-tuned\end{tabular}}} \\ \midrule
\textbf{ChemProt}                                      & Micro F-1                                             & 79.1 (0.4)                                                                                       & \textbf{80.3 (0.1)}                                                                            & 79.0 (0.2)                                                                                       & 79.1 (0.5)                                                                              \\
\textbf{}                                              & Macro F-1                                             & 52.1 (0.5)                                                                                       & 51.6 (0.6)                                                                                     & 51.6 (0.4)                                                                                       & \textbf{52.6 (0.3)}                                                                     \\
\textbf{SciCite}                                       & Micro F-1                                             & 85.7 (0.1)                                                                                       & 85.6 (0.1)                                                                                     & \textbf{85.8 (0.1)}                                                                              & 85.5 (0.1)                                                                              \\
\textbf{}                                              & Macro F-1                                             & \textbf{84.3 (0.1)}                                                                              & 84.1 (0.1)                                                                                     & 84.2 (0.1)                                                                                       & 84.0 (0.1)                                                                              \\
\textbf{SciERC-Rel}                                    & Micro F-1                                             & 84.3 (0.3)                                                                                       & 84.5 (0.3)                                                                                     & \textbf{84.6 (0.2)}                                                                              & 83.5 (0.4)                                                                              \\
\textbf{}                                              & Macro F-1                                             & 74.1 (0.7)                                                                                       & \textbf{74.9 (0.7)}                                                                            & 74.6 (0.4)                                                                                       & 72.9 (0.7)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Text Classification\\ Average Score\end{tabular}}} & 76.6                                                                                             & \textbf{76.8}                                                                                  & 76.6                                                                                             & 76.3                                                                                    \\ \midrule
\textbf{bc5cdr}                                        & Micro F-1                                             & 97.0 (0.0)                                                                                       & 97.0 (0.0)                                                                                     & 96.9 (0.0)                                                                                       & \textbf{97.2 (0.0)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 88.3 (0.0)                                                                                       & 88.3 (0.1)                                                                                     & 87.9 (0.0)                                                                                       & \textbf{88.7 (0.1)}                                                                     \\
\textbf{JNLPBA}                                        & Micro F-1                                             & 93.4 (0.1)                                                                                       & \textbf{93.5 (0.0)}                                                                            & 93.4 (0.0)                                                                                       & \textbf{93.5 (0.0)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 78.0 (0.3)                                                                                       & \textbf{78.6 (0.1)}                                                                            & 77.9 (0.1)                                                                                       & 78.5 (0.1)                                                                              \\
\textbf{NCBI-disease}                                  & Micro F-1                                             & \textbf{98.2 (0.0)}                                                                              & 98.0 (0.0)                                                                                     & 98.1 (0.0)                                                                                       & \textbf{98.2 (0.0)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & \textbf{91.4 (0.1)}                                                                              & 90.5 (0.1)                                                                                     & 90.7 (0.1)                                                                                       & 91.3 (0.1)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}NER Average \\ Score\end{tabular}}}                & 91.1                                                                                             & 91                                                                                             & 90.8                                                                                             & \textbf{91.2}                                                                           \\ \midrule
\textbf{TriviaQA}                                      & Micro F-1                                             & 62.9 (0.1)                                                                                       & 61.4 (0.1)                                                                                     & 59.1 (0.1)                                                                                       & \textbf{63.6 (0.1)}                                                                     \\
                                                       & Macro F-1                                             & 66.2 (0.1)                                                                                       & 64.7 (0.1)                                                                                     & 62.4 (0.1)                                                                                       & \textbf{66.8 (0.1)}                                                                     \\
\textbf{SQuAD}                                         & Micro F-1                                             & 76.6 (0.1)                                                                                       & 76.3 (0.1)                                                                                     & 72.5 (0.1)                                                                                       & \textbf{77.1 (0.1)}                                                                     \\
                                                       & Macro F-1                                             & 85.1 (0.1)                                                                                       & 84.8 (0.0)                                                                                     & 82.3 (0.1)                                                                                       & \textbf{85.4 (0.0)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}QA Average\\ Score\end{tabular}}}                  & 72.7                                                                                             & 71.8                                                                                           & 69.1                                                                                             & \textbf{73.2} \\ \bottomrule                                                                         
\end{tabular}
\caption{DistilBERT Results for Reduced Models. \textbf{Bold} indicates the best average score between the reduced and fully fine-tuned versions of each model. Each score represents the average score of 10 runs, with the standard errors for each score in parentheses.}
\label{tab:distilbert}
\end{table*}

==> submissions/TMLR August 2022/Early_Exiting_Results.tex <==
\begin{table*}[ht]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lcccccccccccccccc}
\toprule
                                                                          & \multicolumn{2}{c}{\textbf{Chemprot}} & \multicolumn{2}{c}{\textbf{SciCite}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}SciERC\\ Rel\end{tabular}}} & \multicolumn{2}{c}{\textbf{bc5cdr}} & \multicolumn{2}{c}{\textbf{JNLPBA}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}NCBI\\ Disease\end{tabular}}} & \multicolumn{2}{c}{\textbf{TriviaQA}} & \multicolumn{2}{c}{\textbf{SQuAD}} \\
                                                                          \cmidrule(l{7pt}r{7pt}){2-3}
                                                                         \cmidrule(l{7pt}r{7pt}){4-5}
                                                                          \cmidrule(l{7pt}r{7pt}){6-7}
                                                                          \cmidrule(l{7pt}r{7pt}){8-9}                                                  \cmidrule(l{7pt}r{7pt}){10-11}\cmidrule(l{7pt}r{7pt}){12-13}\cmidrule(l{7pt}r{7pt}){14-15}\cmidrule(l{7pt}r{7pt}){16-17}
                        
                        
                        
                        & F1                & Time              & F1               & Time              & F1                                      & Time                                    & F1               & Time             & F1               & Time             & F1                                       & Time                                     & F1                & Time              & F1              & Time             \\ \midrule
\multicolumn{17}{c}{\textbf{RoBERTa-Large}}                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
Baseline                                                                  & 84.3              & 76s               & 85.0             & 36s               & 80.2                                    & 17s                                     & 90.0             & 14min            & 79.4             & 12min            & 93                                       & 148s                                     & 78.2              & 55min             & 91.8            & 34min            \\ \cmidrule(l{7pt}r{7pt}){2-17} 
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Early \\ Exiting\end{tabular}} & -0.1              & -29\%             & 0.0              & -27\%             & 0.0                                     & -16\%                                   & -0.1             & -20\%            & -0.2             & -11\%            & 0.0                                      & -31\%                                    & -0.1              & -7\%              & -0.1            & -4\%             \\
                                                                          & -0.5              & -32\%             & -0.4             & -30\%             & -0.3                                    & -20\%                                   & -0.2             & -28\%            & -0.4             & -16\%            & -0.3                                     & -38\%                                    & -2.0              & -13\%             & -0.4            & -10\%            \\
                                                                          & -1.5              & 38\%              & -0.8             & -35\%             & -0.7                                    & -25\%                                   & -1.5             & -39\%            & -0.9             & -25\%            & -1.5                                     & -44\%                                    & -3.2              & -14\%             & -1.4            & -15\%            \\ \midrule
\multicolumn{17}{c}{\textbf{DeBERTa V2 XL}}                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \midrule
Baseline                                                                  & 86.8              & 131s              & 85.2             & 67s               & 79.9                                    & 30s                                     & 91.3             & 24min            & 78.5             & 22min            & 93.3                                     & 252s                                     & 80.6              & 94min             & 94.5            & 59min            \\ \cmidrule(l{7pt}r{7pt}){2-17}
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Early \\ Exiting\end{tabular}} & -0.4              & -10\%             & -0.3             & -15\%             & -0.6                                    & -9\%                                    & -0.1             & -4\%             & -0.1             & -2\%             & -0.2                                     & -5\%                                     & 0.0               & -5\%              & 0.0             & -4\%             \\
                                                                          & -0.8              & -14\%             & -0.6             & -18\%             & -0.8                                    & -16\%                                   & -3.2             & -12\%            & -0.3             & -3\%             & -5.4                                     & -31\%                                    & -0.8              & -7\%              & -2.0            & -9\%             \\
                                                                          & -1.5              & -18\%             & -1.4             & -22\%             & -1.0                                    & -21\%                                   & -36.1            & -47\%            & -35.0            & -45\%            & -16.3                                    & -48\%                                    & -3.4              & -11\%             & -3.3            & -12\% \\ \bottomrule           
\end{tabular}
\caption{Inference times comparison between baseline models and their reduced configurations using early exiting. For our top two performing models, RoBERTa-Large and DeBERTa V2 XL, we explored how embedding recycling could be paired with another efficiency technique, early exiting \citep{xin2020deebert}. For our early exiting testing, we used reduced models in which the earlier half of the transformer layers were removed and cached. Each column indicates varies tradeoffs between loss in F1 score and inference speedup. The percentage time improvements solely indicate inference time gains from early exiting before adding gains from embedding recycling. \jon{Review this caption}}
\label{tab:early_exiting}
\end{table*}

==> submissions/TMLR August 2022/HalfPrecision.tex <==



\begin{table*}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4.6pt}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
                                                                                            & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}RoBERTa \\ Large\end{tabular}}                                                                                                            & \multicolumn{3}{c}{(Sci)BERT}                    
                                                                                            \\ 
                                                                                            \cmidrule(l{7pt}r{7pt}){2-4} \cmidrule(l{7pt}r{7pt}){5-7}
Task                                                                               & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Adpt\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Adpt\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}       \\ 
\midrule
 
ChemProt                                                                           & 84.3 & 84.1 & 83.9 & 84.0 & 84.2 & 84.1                         \\
SciCite                                                                            & 85.0 & 82.5 & 85.5 & 86.6 & 85.5 & 86.0                          \\
SciERC-Rel                                                                        & 80.2 & 85.7 & 80.5 & 76.7 & 86.0 & 79.8                           \\ \hdashline[1pt/1pt]
Classification Avg. & 83.2 & 84.1 & 83.3 & 82.4 & 85.2 & 83.3                        \\ \midrule
bc5cdr                                                                           & 90.0 & 90.0 & 90.4 & 90.7 & 90.0 & 91.3                 \\
JNLPBA                                                                            & 79.4 & 79.1 & 78.7  & 78.8 & 79.9 & 79.0                           \\
NCBI-disease                                                                       & 93.0 & 92.8 & 93.2 & 93.4 & 93.1  & 92.9                  \\ \hdashline[1pt/1pt]
NER Avg.                & 87.5 & 87.3 & 87.4 & 87.7 & 87.6 & 87.7      \\ \midrule
TriviaQA         & 78.2 & 78.5 & 79.8 & 67.4 & 67.4 & 69.1                 \\
SQuAD       & 91.8 & 93.5 & 93.6 & 87.5 & 87.9 & 88.4                 \\ \hdashline[1pt/1pt]
\begin{tabular}[c]{@{}l@{}}QA Avg.\end{tabular} & 85.0 & 86.0 & 86.7 & 77.5 & 77.6 & 78.8  \\ \bottomrule          
\end{tabular}
\caption{Half Precision Inference Results for Embedding Recycling. After training using full precision, we run inference for the reduced (Rdc), adapter-based (Adpt), and fully fine-tuned (Full) configurations of the RoBERTa and SciBERT models using half-precision storage. The reduced configuration corresponds to layer recycling on a reduced transformer model. The adapter-based configuration corresponds to layer recycling on a reduced frozen transformer model with added trainable Adapter modules. We find that half-precision has a negligible effect on F1-scores at inference. Error propagation rarely changes the calculated scores and when it does, it only changes rounding at the tenth decimal place. Each score represents the average score of 5 runs.
}
\label{tab:halfprecision}
\end{table*}

==> submissions/TMLR August 2022/MiniLM_384_Semifrozen.tex <==


\begin{table*}[ht]
\centering
\begin{tabular}{llrrrr}
\toprule
                                                       &                                                       & \multicolumn{4}{c}{\textbf{MiniLM: L6-H384}}                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
                                                       & \textbf{}                                  & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}2 Layers \\ Reduced\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}3 Layers \\ Reduced\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}4 Layers \\ Reduced\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Fully \\ Fine-tuned\end{tabular}}} \\ \midrule
\textbf{ChemProt}                                      & Micro F-1                                             & 75.4 (0.5)                                                                                       & \textbf{76.9 (0.2)}                                                                            & 74.9 (0.3)                                                                                       & 74.6 (0.4)                                                                              \\
\textbf{}                                              & Macro F-1                                             & 47.3 (0.7)                                                                                       & \textbf{50.4 (0.2)}                                                                            & 48.8 (0.4)                                                                                       & 47.1 (0.8)                                                                              \\
\textbf{SciCite}                                       & Micro F-1                                             & 84.4 (0.1)                                                                                       & \textbf{85.4 (0.1)}                                                                            & 85.1 (0.1)                                                                                       & 84.4 (0.1)                                                                              \\
\textbf{}                                              & Macro F-1                                             & 82.8 (0.1)                                                                                       & \textbf{83.7 (0.1)}                                                                            & 83.4 (0.1)                                                                                       & 82.8 (0.1)                                                                              \\
\textbf{SciERC-Rel}                                    & Micro F-1                                             & 83.2 (0.3)                                                                                       & 82.6 (0.3)                                                                                     & \textbf{83.3 (0.2)}                                                                              & 79.5 (0.9)                                                                              \\
\textbf{}                                              & Macro F-1                                             & 72.7 (0.6)                                                                                       & 72.1 (0.6)                                                                                     & \textbf{73.7 (0.3)}                                                                              & 68.9 (1.1)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Text Classification\\ Average Score\end{tabular}}} & 74.3                                                                                             & \textbf{75.2}                                                                                  & 74.9                                                                                             & 72.9                                                                                    \\ \midrule
\textbf{bc5cdr}                                        & Micro F-1                                             & 96.6 (0.0)                                                                                       & 96.3 (0.0)                                                                                     & 95.6 (0.0)                                                                                       & \textbf{96.9 (0.0)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 86.9 (0.1)                                                                                       & 85.9 (0.1)                                                                                     & 83.2 (0.1)                                                                                       & \textbf{88.3 (0.1)}                                                                     \\
\textbf{JNLPBA}                                        & Micro F-1                                             & 93.0 (0.0)                                                                                       & 92.2 (0.0)                                                                                     & 92.0 (0.0)                                                                                       & \textbf{93.3 (0.0)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 76.3 (0.1)                                                                                       & 74.0 (0.1)                                                                                     & 73.6 (0.1)                                                                                       & \textbf{77.2 (0.1)}                                                                     \\
\textbf{NCBI-disease}                                  & Micro F-1                                             & 98.0 (0.0)                                                                                       & 97.9 (0.0)                                                                                     & 97.7 (0.0)                                                                                       & \textbf{98.2 (0.0)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 90.6 (0.1)                                                                                       & 89.9 (0.1)                                                                                     & 88.9 (0.1)                                                                                       & \textbf{91.7 (0.1)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}NER Average \\ Score\end{tabular}}}                & 90.2                                                                                             & 89.4                                                                                           & 88.5                                                                                             & \textbf{90.9}                                                                           \\ \midrule
\textbf{TriviaQA}                                      & Micro F-1                                             & 66.6 (0.1)                                                                                       & 65.6 (0.1)                                                                                     & 63.4 (0.1)                                                                                       & \textbf{67.6 (0.2)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 69.9 (0.1)                                                                                       & 69.2 (0.1)                                                                                     & 67.0 (0.1)                                                                                       & \textbf{71.0 (0.2)}                                                                     \\
\textbf{SQuAD}                                         & Micro F-1                                             & \textbf{81.6 (0.0)}                                                                              & 80.9 (0.1)                                                                                     & 74.2 (0.2)                                                                                       & \textbf{81.6 (0.1)}                                                                     \\
                                                       & Macro F-1                                             & \textbf{89.7 (0.0)}                                                                              & 89.0 (0.0)                                                                                     & 84.5 (0.1)                                                                                       & 89.6 (0.0)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}QA Average\\ Score \end{tabular}}}                  & 76.9                                                                                             & 76.2                                                                                           & 72.3                                                                                             & \textbf{77.4}    \\ \bottomrule                                                                      
\end{tabular}
\caption{MiniLM L6-H384 Results for Reduced Models. \textbf{Bold} indicates the best average score between the reduced and fully fine-tuned versions of each model. Each score represents the average score of 10 runs, with the standard errors for each score in parentheses.}
\label{tab:minilm_384}
\end{table*}

==> submissions/TMLR August 2022/MiniLM_768_Semifrozen.tex <==


\begin{table*}[ht]
\centering
\begin{tabular}{llrrrr}
\toprule
                                                       &                                                       & \multicolumn{4}{c}{\textbf{MiniLM: 6L-H768}}                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
                                                       & \textbf{}                                  & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}2 Layers \\ Reduced\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}3 Layers \\ Reduced\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}4 Layers \\ Reduced\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Fully \\ Fine-tuned\end{tabular}}} \\ \midrule
\textbf{ChemProt}                                      & Micro F-1                                             & \textbf{79.4 (0.3)}                                                                              & 78.3 (0.4)                                                                                     & 79.0 (0.2)                                                                                       & 79.3 (0.3)                                                                              \\
\textbf{}                                              & Macro F-1                                             & 51.8 (0.4)                                                                                       & 50.6 (0.4)                                                                                     & 52.0 (0.2)                                                                                       & \textbf{52.6 (0.4)}                                                                     \\
\textbf{SciCite}                                       & Micro F-1                                             & 85.4 (0.1)                                                                                       & 85.8 (0.2)                                                                                     & 85.9 (0.1)                                                                                       & \textbf{86.0 (0.2)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 84.1 (0.2)                                                                                       & 84.5 (0.2)                                                                                     & 84.5 (0.1)                                                                                       & \textbf{84.6 (0.2)}                                                                     \\
\textbf{SciERC-Rel}                                    & Micro F-1                                             & 84.7 (0.3)                                                                                       & 83.9 (0.3)                                                                                     & 84.1 (0.4)                                                                                       & \textbf{86.3 (0.2)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 75.0 (0.4)                                                                                       & 74.8 (0.4)                                                                                     & 75.3 (0.6)                                                                                       & \textbf{78.2 (0.6)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Text Classification\\ Average Score\end{tabular}}} & 76.7                                                                                             & 76.3                                                                                           & 76.8                                                                                             & \textbf{77.8}                                                                           \\ \midrule
\textbf{bc5cdr}                                        & Micro F-1                                             & 96.1 (0.3)                                                                                       & \textbf{96.8 (0.0)}                                                                            & 96.6 (0.0)                                                                                       & \textbf{96.8 (0.2)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 84.6 (1.1)                                                                                       & \textbf{87.8 (0.1)}                                                                            & 86.6 (0.0)                                                                                       & 87.5 (1.0)                                                                              \\
\textbf{JNLPBA}                                        & Micro F-1                                             & 93.2 (0.0)                                                                                       & 93.2 (0.0)                                                                                     & \textbf{93.3 (0.0)}                                                                              & \textbf{93.3 (0.0)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & \textbf{77.5 (0.1)}                                                                              & 77.3 (0.1)                                                                                     & 77.3 (0.1)                                                                                       & 76.9 (0.2)                                                                              \\
\textbf{NCBI-disease}                                  & Micro F-1                                             & \textbf{98.3 (0.0)}                                                                              & 98.2 (0.0)                                                                                     & 98.2 (0.0)                                                                                       & \textbf{98.3 (0.0)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & \textbf{92.1 (0.1)}                                                                              & 91.1 (0.1)                                                                                     & 91.0 (0.1)                                                                                       & \textbf{92.1 (0.1)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}NER Average \\ Score \end{tabular}}}                & 90.3                                                                                             & 90.7                                                                                           & 90.5                                                                                             & \textbf{90.8}                                                                           \\ \midrule
\textbf{TriviaQA}                                      & Micro F-1                                             & 70.2 (0.1)                                                                                       & 68.9 (0.1)                                                                                     & 65.5 (0.1)                                                                                       & \textbf{70.4 (0.2)}                                                                     \\
                                                       & Macro F-1                                             & 73.4 (0.1)                                                                                       & 72.2 (0.1)                                                                                     & 68.9 (0.1)                                                                                       & \textbf{73.8 (0.2)}                                                                     \\
\textbf{SQuAD}                                         & Micro F-1                                             & 77.6 (0.1)                                                                                       & 75.6 (0.1)                                                                                     & 65.4 (0.2)                                                                                       & \textbf{78.9 (0.1)}                                                                     \\
                                                       & Macro F-1                                             & 86.4 (0.1)                                                                                       & 85.0 (0.1)                                                                                     & 77.0 (0.1)                                                                                       & \textbf{87.0 (0.1)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}QA Average\\ Score\end{tabular}}}                  & 76.9                                                                                             & 75.4                                                                                           & 69.2                                                                                             & \textbf{77.5}  \\ \bottomrule                                                                        
\end{tabular}
\caption{MiniLM L6-H768 Results for Reduced Models. \textbf{Bold} indicates the best average score between the reduced and fully fine-tuned versions of each model. Each score represents the average score of 10 runs, with the standard errors for each score in parentheses.}
\label{tab:minilm_768}
\end{table*}

==> submissions/TMLR August 2022/NLI_Results.tex <==

\begin{table*}[ht]
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{lrrrr}
\toprule
                                                                         & \multicolumn{4}{c}{\textbf{DeBERTa V2 XL}}                                                                                                                                                                     \\ \midrule
                                                                         & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Rdc +\\ Half\\ Adpt\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Full\\ Adpt\end{tabular}} & \multicolumn{1}{l}{Rdc} & \multicolumn{1}{l}{Full} \\ \midrule
CoLA                                                                     & 70.9                                                                            & 71.3                                                                    & 70.8                    & 71.2                     \\
SST-2                                                                    & 96.9                                                                            & 97.1                                                                    & 97.1                    & 97.4                     \\ \hdashline[1pt/1pt]
\begin{tabular}[c]{@{}l@{}}Single\\ Sentence Avg.\end{tabular}           & 83.9                                                                            & \textbf{84.2}                                                           & 84.0                    & \textbf{84.3}            \\  \midrule
MRPC                                                                     & 93.9                                                                            & 94.0                                                                    & 93.4                    & 93.9                     \\
STS-B                                                                    & 92.4                                                                            & 92.7                                                                    & 92.5                    & 92.8                     \\ \hdashline[1pt/1pt]
\begin{tabular}[c]{@{}l@{}}Similarity and\\ Paraphrase Avg.\end{tabular} & 93.2                                                                            & \textbf{93.4}                                                           & 93.0                    & \textbf{93.4}            \\ \midrule
MNLI                                                                     & 91.6                                                                            & 92.0                                                                    & 91.0                    & 91.4                     \\
QNLI                                                                     & 95.0                                                                            & 95.1                                                                    & 94.1                    & 94.8                     \\ \hdashline[1pt/1pt]
NLI Avg.                                                                 & 93.3                                                                            & \textbf{93.6}                                                           & 92.6                    & \textbf{93.1} \\ \midrule          
\end{tabular}
\caption{Test scores of reduced (Rdc) and reduced adapter (Rdc + Half Adpt) models on the GLUE tasks for DeBERTa V2 XL. \textbf{Bold} indicates the best average score between the reduced and fully fine-tuned (Full) versions for both the standard and adapter-based configurations. Each score represents the average macro F-1 score of 5 runs. Our results for MNLI correspond to MNLI-matched. For MRPC, MNLI, and QNLI, we report the macro F1 scores. For CoLA, we report the Matthews correlation coefficient (MCC). For SST-2, we report the accuracy. For STS-B, we report the Pearson's correlation coefficient. }
\end{table*}

==> submissions/TMLR August 2022/RoBERTa_Semifrozen.tex <==


\begin{table*}[htp]
\centering
\small
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{llrrrrrr}
\toprule
                                                          &                                              & \multicolumn{1}{l}{}                                                                      & \multicolumn{1}{l}{}                                                                      & \multicolumn{4}{c}{\textbf{RoBERTa-Large}}                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
                                                          & \textbf{}                                    & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Reduced +\\ Half Adpt\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Full \\ Adapters\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}6 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}12 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}18 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Fully \\ Finetuned\end{tabular}}} \\ \midrule
\textbf{ChemProt}                                         & Micro F-1                                    & 84.1 (0.4)                                                                                & \textbf{85.2 (0.3)}                                                                       & 84.2 (0.3)                                                                                     & 84.3 (0.2)                                                                                      & 82.0 (0.2)                                                                                      & 83.9 (0.3)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & \textbf{60.8 (0.7)}                                                                       & 57.5 (0.7)                                                                                & 56.4 (0.4)                                                                                     & 56.5 (0.3)                                                                                      & 54.5 (0.5)                                                                                      & 56.5 (0.4)                                                                              \\
\textbf{SciCite}                                          & Micro F-1                                    & 85.2 (0.3)                                                                                & 85.6 (0.5)                                                                                & 86.2 (0.2)                                                                                     & 86.2 (0.2)                                                                                      & 86.2 (0.2)                                                                                      & \textbf{86.8 (0.2)}                                                                     \\
\textbf{}                                                 & Macro F-1                                    & 82.4 (0.4)                                                                                & 82.9 (0.6)                                                                                & 84.9 (0.2)                                                                                     & 85.0 (0.2)                                                                                      & 85.0 (0.2)                                                                                      & \textbf{85.5 (0.2)}                                                                     \\
\textbf{SciERC-Rel}                                       & Micro F-1                                    & 89.0 (0.5)                                                                                & \textbf{89.3 (0.6)}                                                                       & 87.1 (0.4)                                                                                     & 86.8 (0.4)                                                                                      & 86.1 (0.2)                                                                                      & 87.3 (0.4)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 85.7 (0.7)                                                                                & \textbf{85.9 (0.9)}                                                                       & 79.4 (0.7)                                                                                     & 80.2 (0.8)                                                                                      & 76.2 (0.4)                                                                                      & 80.4 (0.6)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Text Classification\\ Average Score\end{tabular}}} & \textbf{81.2}                                                                             & 81.1                                                                                      & 79.7                                                                                           & 79.8                                                                                            & 78.3                                                                                            & 80.1                                                                                    \\ \midrule
\textbf{bc5cdr}                                           & Micro F-1                                    & 97.4 (0.0)                                                                                & \textbf{97.6 (0.0)}                                                                       & 97.2 (0.3)                                                                                     & 97.4 (0.0)                                                                                      & 97.3 (0.0)                                                                                      & 97.5 (0.0)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 90.0 (0.0)                                                                                & \textbf{90.6 (0.0)}                                                                       & 89.0 (1.2)                                                                                     & 90.0 (0.0)                                                                                      & 89.5 (0.1)                                                                                      & 90.4 (0.1)                                                                              \\
\textbf{JNLPBA}                                           & Micro F-1                                    & 93.8 (0.0)                                                                                & 93.8 (0.0)                                                                                & 93.8 (0.0)                                                                                     & \textbf{93.9 (0.0)}                                                                             & 93.7 (0.0)                                                                                      & 93.7 (0.1)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 79.1 (0.1)                                                                                & 79.2 (0.2)                                                                                & 79.3 (0.1)                                                                                     & \textbf{79.4 (0.1)}                                                                             & 79.0 (0.1)                                                                                      & 78.7 (0.3)                                                                              \\
\textbf{NCBI-disease}                                     & Micro F-1                                    & 98.5 (0.0)                                                                                & \textbf{98.6 (0.0)}                                                                       & 98.5 (0.0)                                                                                     & 98.5 (0.0)                                                                                      & 98.4 (0.0)                                                                                      & \textbf{98.6 (0.0)}                                                                     \\
\textbf{}                                                 & Macro F-1                                    & 92.8 (0.1)                                                                                & 93.1 (0.1)                                                                                & 93.0 (0.1)                                                                                     & 93.0 (0.1)                                                                                      & 92.4 (0.1)                                                                                      & \textbf{93.2 (0.1)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}NER Average \\ Score\end{tabular}}}                & 91.9                                                                                      & \textbf{92.1}                                                                             & 91.8                                                                                           & 92.0                                                                                            & 91.7                                                                                            & 92.0                                                                                    \\ \midrule
\textbf{TriviaQA}                                         & Micro F-1                                    & 75.3 (0.1)                                                                                & \textbf{76.8 (0.2)}                                                                       & 76.6 (0.2)                                                                                     & 75.1 (0.1)                                                                                      & 70.8 (0.1)                                                                                      & 76.7 (0.1)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 78.5 (0.1)                                                                                & \textbf{79.8 (0.1)}                                                                       & 79.7 (0.2)                                                                                     & 78.2 (0.1)                                                                                      & 73.8 (0.1)                                                                                      & \textbf{79.8 (0.1)}                                                                     \\
\textbf{SQuAD}                                            & Micro F-1                                    & 87.0 (0.1)                                                                                & 86.7 (0.0)                                                                                & 86.2 (0.0)                                                                                     & 84.7 (0.0)                                                                                      & 79.3 (0.0)                                                                                      & \textbf{87.4 (0.0)}                                                                     \\
                                                          & Macro F-1                                    & 93.5 (0.1)                                                                                & 93.4 (0.0)                                                                                & 92.8 (0.0)                                                                                     & 91.8 (0.0)                                                                                      & 87.8 (0.0)                                                                                      & \textbf{93.6 (0.0)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}QA Average\\ Score\end{tabular}}}                  & 83.6                                                                                      & 84.1                                                                                      & 83.8                                                                                           & 82.4                                                                                            & 77.9                                                                                            & \textbf{84.3} \\ \bottomrule                                                                         
\end{tabular}
\caption{RoBERTa Results for Reduced Models. \textbf{Bold} indicates the best average score between the standard reduced, adapter-based reduced, and fully fine-tuned versions of each model. \textbf{Reduced + Half Adpt} indicates adapters on the transformer layers of a fully frozen reduced model, where the earlier half of transformer layers were removed and their activations cached. \textbf{Full Adapters} indicates adapters on all transformer layers of a fully frozen model. Each score represents the average score of 10 runs, with the standard errors for each score in parentheses.}
\label{tab:roberta}
\end{table*}

==> submissions/TMLR August 2022/SciBERT_Semifrozen.tex <==


\begin{table*}[htp]
\centering
\small
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{llrrrrrr}
\toprule
                                                       &                                                       & \multicolumn{1}{l}{}                                                                      & \multicolumn{1}{l}{}                                                                      & \multicolumn{4}{c}{\textbf{SciBERT}}                                                                                                                                                                                                                                                                                                                                                       \\ \midrule
                                                       &                                 & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Reduced +\\ Half Adpt\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Full \\ Adapters\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}3 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}6 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}9 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Fully \\ Finetuned\end{tabular}}} \\ \midrule
\textbf{ChemProt}                                      & Micro F-1                                             & 84.2 (0.3)                                                                                & \textbf{84.9 (0.4)}                                                                       & 83.8 (0.4)                                                                                     & 84.0 (0.2)                                                                                     & 81.9 (0.2)                                                                                     & 84.0 (0.3)                                                                              \\
\textbf{}                                              & Macro F-1                                             & 56.9 (0.8)                                                                                & 54.8 (0.4)                                                                                & 56.5 (0.5)                                                                                     & \textbf{57.0 (0.3)}                                                                            & 54.3 (0.3)                                                                                     & 56.3 (0.4)                                                                              \\
\textbf{SciCite}                                       & Micro F-1                                             & 86.6 (0.2)                                                                                & 85.8 (0.1)                                                                                & 87.1 (0.1)                                                                                     & \textbf{87.6 (0.1)}                                                                            & 87.4 (0.1)                                                                                     & 87.1 (0.2)                                                                              \\
\textbf{}                                              & Macro F-1                                             & 85.5 (0.3)                                                                                & 84.6 (0.1)                                                                                & 86.1 (0.1)                                                                                     & \textbf{86.6 (0.1)}                                                                            & 86.2 (0.1)                                                                                     & 86.0 (0.2)                                                                              \\
\textbf{SciERC-Rel}                                    & Micro F-1                                             & \textbf{89.4 (0.4)}                                                                       & 88.5 (0.6)                                                                                & 86.6 (0.3)                                                                                     & 86.1 (0.2)                                                                                     & 85.4 (0.2)                                                                                     & 86.3 (0.2)                                                                              \\
\textbf{}                                              & Macro F-1                                             & \textbf{86.0 (0.7)}                                                                       & 85.5 (0.6)                                                                                & 77.6 (0.5)                                                                                     & 76.7 (0.3)                                                                                     & 76.2 (0.4)                                                                                     & 79.8 (0.5)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Text Classification\\ Average Performance\end{tabular}}} & \textbf{81.4}                                                                             & 80.7                                                                                      & 79.6                                                                                           & 79.7                                                                                           & 78.6                                                                                           & 79.9                                                                                    \\ \midrule
\textbf{bc5cdr}                                        & Micro F-1                                             & 97.5 (0.0)                                                                                & \textbf{97.7 (0.1)}                                                                       & 97.7 (0.0)                                                                                     & 97.6 (0.0)                                                                                     & 97.5 (0.0)                                                                                     & \textbf{97.7 (0.0)}                                                                     \\
\textbf{}                                              & Macro F-1                                             & 90.0 (0.0)                                                                                & 90.9 (0.1)                                                                                & 91.0 (0.1)                                                                                     & 90.7 (0.0)                                                                                     & 90.2 (0.1)                                                                                     & \textbf{91.3 (0.0)}                                                                     \\
\textbf{JNLPBA}                                        & Micro F-1                                             & \textbf{94.0 (0.0)}                                                                       & 93.5 (0.0)                                                                                & 93.6 (0.1)                                                                                     & 93.7 (0.1)                                                                                     & 93.8 (0.0)                                                                                     & 93.6 (0.1)                                                                              \\
\textbf{}                                              & Macro F-1                                             & \textbf{79.8 (0.0)}                                                                       & 78.3 (0.2)                                                                                & 78.6 (0.4)                                                                                     & 78.8 (0.2)                                                                                     & 79.0 (0.1)                                                                                     & 79.0 (0.2)                                                                              \\
\textbf{NCBI-disease}                                  & Micro F-1                                             & \textbf{98.6 (0.0)}                                                                       & 98.5 (0.0)                                                                                & 98.5 (0.0)                                                                                     & \textbf{98.6 (0.0)}                                                                            & 98.5 (0.0)                                                                                     & 98.5 (0.0)                                                                              \\
\textbf{}                                              & Macro F-1                                             & 93.1 (0.1)                                                                                & 93.0 (0.1)                                                                                & 92.9 (0.1)                                                                                     & \textbf{93.4 (0.1)}                                                                            & 93.1 (0.1)                                                                                     & 92.9 (0.1)                                                                              \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}NER Average\\ Perforamcne\end{tabular}}}                 & \textbf{92.2}                                                                             & 92.0                                                                                      & 92                                                                                             & 92.1                                                                                           & 92                                                                                             & \textbf{92.2}  \\ \bottomrule                                                                        
\end{tabular}
\caption{SciBERT text classification and NER results for Reduced Models. \textbf{Bold} indicates the best average score between the standard reduced, adapter-based reduced, and fully fine-tuned versions of each model. \textbf{Reduced + Half Adpt} indicates adapters on the transformer layers of a fully frozen reduced model, where the earlier half of transformer layers were removed and their activations cached. \textbf{Full Adapters} indicates adapters on all transformer layers of a fully frozen model. Each score represents the average score of 10 runs, with the standard errors for each score in parentheses. QA tasks are not included since SciBERT was pretrained for scientific datasets.}
\label{tab:scibert}
\end{table*}
















\begin{table*}[htp]
\centering
\small
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{llrrrrrr}
\toprule
                                                &                                        & \multicolumn{6}{c}{\textbf{BERT}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \midrule
                                                &                                        & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Reduced +\\ Half Adpt\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Full \\ Adapters\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}3 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}6 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}9 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Fully \\ Finetuned\end{tabular}}} \\ \midrule
\textbf{TriviaQA}                               & Micro F-1                              & 63.9 (0.5)                                                                                & 65.5 (0.1)                                                                                & 65.7 (0.1)                                                                                     & 64.1 (0.2)                                                                                     & 61.4 (0.1)                                                                                     & \textbf{66.0 (0.1)}                                                                     \\
\textbf{}                                       & Macro F-1                              & 67.4 (0.5)                                                                                & 68.9 (0.1)                                                                                & 68.9 (0.1)                                                                                     & 67.4 (0.1)                                                                                     & 64.8 (0.1)                                                                                     & \textbf{69.1 (0.1)}                                                                     \\
\textbf{SQuAD}                                  & Micro F-1                              & 80.2 (0.1)                                                                                & 80.2 (0.0)                                                                                & 80.8 (0.1)                                                                                     & 79.5 (0.1)                                                                                     & 75.4 (0.1)                                                                                     & \textbf{81.1 (0.1)}                                                                     \\
\textbf{}                                       & Macro F-1                              & 87.9 (0.1)                                                                                & 87.9 (0.0)                                                                                & 88.4 (0.1)                                                                                     & 87.5 (0.1)                                                                                     & 84.8 (0.1)                                                                                     & \textbf{88.5 (0.0)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}QA Average\\ Scores\end{tabular}}} & 74.9                                                                                      & 75.6                                                                                      & 76.0                                                                                           & 74.6                                                                                           & 71.6                                                                                           & \textbf{76.2}        \\ \midrule                                                                  
\end{tabular}
\caption{BERT QA Results for Reduced Models. \textbf{Bold} indicates the best average score between the standard reduced, adapter-based reduced, and fully fine-tuned versions of each model. \textbf{Reduced + Half Adpt} indicates adapters on the transformer layers of a fully frozen reduced model, where the earlier half of transformer layers were removed and their activations cached. \textbf{Full Adapters} indicates adapters on all transformer layers of a fully frozen model. Each score represents the average score of 10 runs, with the standard errors for each score in parentheses.}
\label{tab:bert}
\end{table*}

==> submissions/TMLR August 2022/T5_Large.tex <==


\begin{table*}[htp]
\centering
\small
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{llrrrrrr}
\toprule
                                                          &                                              & \multicolumn{1}{l}{}                                                                      & \multicolumn{1}{l}{}                                                                       & \multicolumn{4}{c}{\textbf{T5 Large}}                                                                                                                                                                                                                                                                                                                                                        \\ \midrule
                                                          & \textbf{}                                    & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Reduced +\\ Half Adpt\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}} Full \\ Adapters\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}6 Layers \\ Frozen \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}12 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}18 Layers \\ Reduced \end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Fully \\ Finetuned\end{tabular}}} \\ \midrule
\textbf{ChemProt}                                         & Micro F-1                                    & 84.3 (0.6)                                                                                & 84.9 (0.6)                                                                                 & 84.7 (0.6)                                                                                     & 84.6 (0.6)                                                                                      & \textbf{85.0 (0.1)}                                                                             & 84.1 (0.8)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 57.2 (0.7)                                                                                & \textbf{58.0 (0.8)}                                                                        & 56.2 (0.7)                                                                                     & 56.2 (0.7)                                                                                      & 57.4 (0.1)                                                                                      & 56.1 (0.7)                                                                              \\
\textbf{SciCite}                                          & Micro F-1                                    & 86.7 (0.3)                                                                                & 86.2 (0.3)                                                                                 & 87.4 (0.2)                                                                                     & 87.6 (0.1)                                                                                      & \textbf{88.0 (0.2)}                                                                             & 86.4 (0.2)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 85.3 (0.4)                                                                                & 84.5 (0.4)                                                                                 & 86.0 (0.2)                                                                                     & 86.3 (0.2)                                                                                      & \textbf{86.9 (0.2)}                                                                             & 84.9 (0.2)                                                                              \\
\textbf{SciERC-Rel}                                       & Micro F-1                                    & 85.6 (0.4)                                                                                & 85.2 (0.1)                                                                                 & 84.3 (0.3)                                                                                     & 86.8 (0.4)                                                                                      & 83.4 (0.7)                                                                                      & \textbf{87.4 (0.5)}                                                                     \\
\textbf{}                                                 & Macro F-1                                    & 76.2 (1.0)                                                                                & 75.6 (0.2)                                                                                 & 73.6 (0.9)                                                                                     & 77.4 (0.7)                                                                                      & 72.2 (1.0)                                                                                      & \textbf{80.2 (1.1)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Text Classification\\ Average Score\end{tabular}}} & 79.2                                                                                      & 79.1                                                                                       & 78.7                                                                                           & 79.8                                                                                            & 78.8                                                                                            & \textbf{79.9}                                                                           \\ \midrule
\textbf{bc5cdr}                                           & Micro F-1                                    & 93.8 (0.6)                                                                                & 95.7 (0.7)                                                                                 & \textbf{97.7 (0.7)}                                                                            & 97.4 (0.3)                                                                                      & 95.4 (0.8)                                                                                      & 97.5 (0.2)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 79.9 (1.0)                                                                                & 85.7 (1.1)                                                                                 & \textbf{91.1 (0.5)}                                                                            & 90.7 (1.1)                                                                                      & 89.3 (1.0)                                                                                      & 89.9 (0.8)                                                                              \\
\textbf{JNLPBA}                                           & Micro F-1                                    & 93.9 (0.4)                                                                                & 93.8 (0.1)                                                                                 & 93.8 (0.0)                                                                                     & 94.0 (0.0)                                                                                      & 93.9 (0.0)                                                                                      & \textbf{94.2 (0.0)}                                                                     \\
\textbf{}                                                 & Macro F-1                                    & 78.8 (0.6)                                                                                & 79.5 (0.2)                                                                                 & 78.8 (0.1)                                                                                     & 79.6 (0.1)                                                                                      & 79.3 (0.0)                                                                                      & \textbf{80.0 (0.0)}                                                                     \\
\textbf{NCBI-disease}                                     & Micro F-1                                    & 97.8 (0.0)                                                                                & 98.5 (0.0)                                                                                 & 98.5 (0.0)                                                                                     & 98.5 (0.0)                                                                                      & 98.4 (0.0)                                                                                      & \textbf{98.6 (0.0)}                                                                     \\
\textbf{}                                                 & Macro F-1                                    & 92.1 (0.2)                                                                                & 92.5 (0.2)                                                                                 & 93.1 (0.1)                                                                                     & 92.8 (0.0)                                                                                      & 92.2 (0.1)                                                                                      & \textbf{93.5 (0.0)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}NER Average \\ Score\end{tabular}}}                & 89.4                                                                                      & 90.9                                                                                       & 92.2                                                                                           & 92.2                                                                                            & 91.4                                                                                            & \textbf{92.3}                                                                           \\ \midrule
\textbf{TriviaQA}                                         & Micro F-1                                    & 68.2 (0.2)                                                                                & \textbf{68.8 (0.2)}                                                                        & 67.0 (0.0)                                                                                     & 66.9 (0.0)                                                                                      & 63.9 (0.0)                                                                                      & 68.7 (0.0)                                                                              \\
\textbf{}                                                 & Macro F-1                                    & 77.0 (0.1)                                                                                & 77.5 (0.1)                                                                                 & 77.5 (0.0)                                                                                     & 77.3 (0.0)                                                                                      & 74.8 (0.0)                                                                                      & \textbf{78.0 (0.0)}                                                                     \\
\textbf{SQuAD}                                            & Micro F-1                                    & 81.2 (0.1)                                                                                & 82.0 (0.1)                                                                                 & 86.6 (0.1)                                                                                     & 86.3 (0.6)                                                                                      & 85.2 (0.4)                                                                                      & \textbf{86.7 (0.4)}                                                                     \\
                                                          & Macro F-1                                    & 90.6 (0.1)                                                                                & 91.0 (0.1)                                                                                 & 93.8 (0.0)                                                                                     & 93.7 (0.3)                                                                                      & 92.8 (0.2)                                                                                      & \textbf{93.9 (0.3)}                                                                     \\ \midrule
\multicolumn{2}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}QA Average\\ Score\end{tabular}}}                  & 79.2                                                                                      & 79.8                                                                                       & 81.2                                                                                           & 81.0                                                                                            & 79.2                                                                                            & \textbf{81.8}     \\ \bottomrule                                                                     
\end{tabular}
\caption{T5 Large Results for Reduced Models. \textbf{Bold} indicates the best average score between the standard reduced, adapter-based reduced, and fully fine-tuned versions of each model. \textbf{Reduced + Half Adpt} indicates adapters on the encoder and decoder transformer layers of a fully frozen reduced model, where the earlier half of the encoder layers were removed and their activations cached. \textbf{Full Adapters} indicates adapters on all encoder and decoder transformer layers of a fully frozen model. Each score represents the average score of 5 runs, with the standard errors for each score in parentheses.}
\label{tab:t5_large}
\end{table*}

==> submissions/TMLR August 2022/TrainingTimes.tex <==

\begin{table}[!htp]
\footnotesize
\centering
\normalsize
\begin{tabular}{lrrr}
\toprule
\multicolumn{1}{c}{\textbf{Task}} & \multicolumn{1}{c}{\textbf{Averages}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}l@{}} Standard \\ Recycling\end{tabular}}} & \textbf{ \begin{tabular}[c]{@{}l@{}} Adapter-Based \\ Recycling\end{tabular}} \\
\midrule
\textbf{Classification} & \begin{tabular}[c]{@{}l@{}} Training Time\end{tabular} & 2204  & 2349 \\
 & \begin{tabular}[c]{@{}l@{}}Epochs\end{tabular} & 38 & 42 \\
\midrule
\textbf{NER} & \begin{tabular}[c]{@{}l@{}} Training Time\end{tabular} & 4269 & 3857  \\
 & \begin{tabular}[c]{@{}l@{}}Epochs\end{tabular} & 43 & 39 \\
\midrule
\textbf{QA} & \begin{tabular}[c]{@{}l@{}} Training Time\end{tabular} & 8252 & 8513 \\
 & \begin{tabular}[c]{@{}l@{}}Epochs\end{tabular} & 6 & 7 \\
\bottomrule
\end{tabular}
\caption{Average Training Times and Epochs for Embedding Recycling (seconds for training time, count for epochs). \textbf{Standard Recycling} corresponds to layer recycling on a reduced transformer model. \textbf{Adapter-Based Recycling} corresponds to layer recycling on a reduced frozen transformer model with added trainable Adapter modules. Training time and epoch averages are the averages across the RoBERTa, BERT, SciBERT, DeBERTa V2 XL, and T5-Large transformer models and the text classification, NER, and QA datasets tested.}
\label{tab:training_times}
\end{table}

==> submissions/TMLR August 2022/adapters_results.tex <==

\begin{table*}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4.6pt}
\begin{tabular}{lrrrrrrrrrrrr}
\toprule
\textbf{}           & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}RoBERTa \\ Large\end{tabular}}                                                                                                                                                            & \multicolumn{3}{c}{(Sci)BERT}                                                                                                                                                               & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}DeBERTa \\ V2 XL \end{tabular}}                                                                                                                   & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}T5\\ Large\end{tabular}}                                                                                                                       \\ \cmidrule(l{7pt}r{7pt}){2-4}
\cmidrule(l{7pt}r{7pt}){5-7}
\cmidrule(l{7pt}r{7pt}){8-10} 
\cmidrule(l{7pt}r{7pt}){11-13}
Task                & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc +\\ Half\\ Adpt\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\\ Adpt\end{tabular}} & \multicolumn{1}{c}{Full} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc +\\ Half\\ Adpt\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\\ Adpt\end{tabular}} & \multicolumn{1}{c}{Full} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc +\\ Half\\ Adpt\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\\ Adpt\end{tabular}} & \multicolumn{1}{c}{Full} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc +\\ Half\\ Adpt\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\\ Adpt\end{tabular}} & \multicolumn{1}{c}{Full} \\ \midrule
ChemProt            & 84.1                                                                            & 85.2                                                                            & 83.9                     & 84.2                                                                            & 84.9                                                                            & 84.0                     & 87.2                                                                            & 86.5                                                                            & 86.7                     & 84.3                                                                            & 84.9                                                                            & 84.1                     \\
SciCite             & 82.4                                                                            & 82.9                                                                            & 85.5                     & 85.5                                                                            & 84.6                                                                            & 86.0                     & 84.6                                                                            & 85.0                                                                            & 84.4                     & 85.3                                                                            & 84.5                                                                            & 84.9                     \\
SciERC-Rel          & 85.7                                                                            & 85.9                                                                            & 80.4                     & 86.0                                                                            & 85.5                                                                            & 79.8                     & 82.9                                                                            & 82.1                                                                            & 80.2                     & 76.2                                                                            & 75.6                                                                            & 80.2                     \\ \hdashline[1pt/1pt]
Classification Avg. & 84.1                                                                            & \textbf{84.7}                                                                   & 83.3                     & \textbf{85.2}                                                                   & 85.0                                                                              & 83.3                     & \textbf{84.9}                                                                   & 84.6                                                                            & 83.8                     & 81.9                                                                            & 81.7                                                                            & \textbf{83.1}            \\ \midrule
bc5cdr              & 90.0                                                                            & 90.6                                                                            & 90.4                     & 90.0                                                                            & 90.9                                                                            & 91.3                     & 90.7                                                                            & 91.1                                                                            & 91.8                     & 79.9                                                                            & 85.7                                                                            & 89.9                     \\
JNLPBA              & 79.1                                                                            & 79.2                                                                            & 78.7                     & 79.8                                                                            & 78.3                                                                            & 79.0                     & 79.3                                                                            & 79.0                                                                            & 78.2                     & 78.8                                                                            & 79.5                                                                            & 80.0                     \\
NCBI-disease        & 92.8                                                                            & 93.1                                                                            & 93.2                     & 93.1                                                                            & 93.0                                                                            & 92.9                     & 93.3                                                                            & 93.5                                                                            & 93.4                     & 92.1                                                                            & 92.5                                                                            & 93.5                     \\ \hdashline[1pt/1pt]
NER Avg.            & 87.3                                                                            & \textbf{87.6}                                                                   & 87.4                     & 87.6                                                                            & 87.4                                                                            & \textbf{87.7}            & 87.8                                                                            & \textbf{87.9}                                                                   & 87.8                     & 83.6                                                                            & 85.9                                                                            & \textbf{87.8}            \\ \midrule
TriviaQA            & 78.5                                                                            & 79.8                                                                            & 79.8                     & 67.4                                                                            & 68.9                                                                            & 69.1                     & 81.6                                                                            & 82.3                                                                            & 81.8                     & 77.0                                                                            & 77.5                                                                            & 78.2                     \\
SQuAD               & 93.5                                                                            & 93.4                                                                            & 93.6                     & 87.9                                                                            & 87.9                                                                            & 88.5                     & 94.7                                                                            & 93.9                                                                            & 94.6                     & 90.6                                                                            & 91.0                                                                            & 93.9                     \\ \hdashline[1pt/1pt]
QA Avg.             & 86.0                                                                            & 86.6                                                                            & \textbf{86.7}            & 77.6                                                                            & 78.4                                                                            & \textbf{78.8}            & 88.1                                                                            & 88.1                                                                            & \textbf{88.2}            & 83.8                                                                            & {84.3}                                                                   & \textbf{85.9} \\ \bottomrule                   
\end{tabular}
\caption{Test scores of reduced adapter (Rdc + Half Adpt) models on the text classification, NER, and QA tasks. \textbf{Bold} indicates the best average score between the reduced adapter, full adapter (Full Adpt), and fully fine-tuned (Full) versions of each model. 
%The reduced Adapter-based models are fully frozen reduced model with trainable Adapters added, where the earlier half of the transformer layers were removed. 
%Full Adpt indicates adapters on all transformer layers of a fully frozen model. 
Each score represents the average macro F-1 score of 10 runs for RoBERTa, BERT, and the distilled models. The F-1 score averages for DeBERTa and T5 were gathered from 5 runs.
The standard errors for each score are shown in corresponding tables in \autoref{sec:experimental_setup}. For the ChemProt dataset, we report the micro F-1 scores instead, following past work \citep{beltagy2019scibert}. For the QA datasets, we use BERT while we use SciBERT for the text classification and NER datasets since it outperforms BERT on these datasets \citep{beltagy2019scibert}.
%For the reduced configurations, the half of the transformer layers closest to the input were frozen from fine-tuning. For adapters configurations (Frz+Adpt), we froze all the transformer layers from fine-tuning but added trainable adapters \cite{houlsby2019parameter} to the latter half of the transformer layers furthest from the input.
}
\label{tab:adapters}
\end{table*}

==> submissions/TMLR August 2022/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> submissions/TMLR August 2022/meta_results_table.tex <==



\begin{table*}[ht]
\small
\centering
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4.6pt}
\begin{tabular}{@{}lrrrrrrrrrrrrrr@{}}
\toprule
                                                                                            & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}RoBERTa \\ Large\end{tabular}}                                                                                                            & \multicolumn{2}{c}{(Sci)BERT} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}DeBERTa \\ V2 XL \end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}T5 \\ Large\end{tabular}}                                                                                                                                                            & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}MiniLM\\ L6-H768\end{tabular}}                          & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}MiniLM\\ L6-H384\end{tabular}}                          & \multicolumn{2}{c}{DistilBERT}                    
                                                                                            \\ 
                                                                                            \cmidrule(l{7pt}r{7pt}){2-3} \cmidrule(l{7pt}r{7pt}){4-5} \cmidrule(l{7pt}r{7pt}){6-7} \cmidrule(l{7pt}r{7pt}){8-9} \cmidrule(l{7pt}r{7pt}){10-11} \cmidrule(l{7pt}r{7pt}){12-13}  \cmidrule(l{7pt}r{7pt}){14-15}
Task                                                                               & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}} \\ 
\midrule
 
ChemProt                                                                           & {84.3}                                                                                                                                         & \multicolumn{1}{r}{83.9}          & 84.0                                                                                                                                       & \multicolumn{1}{r}{84.0}  & 86.8 & 86.7 & 84.6 & 84.1    & 78.3                                                                      & \multicolumn{1}{r}{{79.3}} & {76.9}                                                             & \multicolumn{1}{r}{74.6}          & {80.3}                                                             & \multicolumn{1}{r}{79.1}                         \\
SciCite                                                                            & 85.0                                                                                                                                                  & \multicolumn{1}{r}{{85.5}} & {86.6}                                                                                                                                         & \multicolumn{1}{r}{86.0} & 85.2 & 84.4 & 86.3 & 84.9   & 84.5                                                                      & \multicolumn{1}{r}{{84.6}} & {83.7}                                                             & \multicolumn{1}{r}{82.8}          & {84.1}                                                             & \multicolumn{1}{r}{84.0}                         \\
SciERC-Rel                                                                        & 80.2                                                                                                                                         & \multicolumn{1}{r}{80.4}          & 76.7                                                                                                                                         & \multicolumn{1}{r}{79.8} & 79.9 & 80.2 & 77.4 & 80.2   & 74.8                                                                      & \multicolumn{1}{r}{{78.2}} & {72.1}                                                             & \multicolumn{1}{r}{68.9}          & {74.9}                                                             & \multicolumn{1}{r}{72.9}                         \\ \hdashline[1pt/1pt]
Classification Avg. & 83.2                                                                                                                                         & \multicolumn{1}{r}{\textbf{83.3}}          & 82.4                                                                                                                                        & \multicolumn{1}{r}{\textbf{83.3}} & \textbf{84.0} & 83.8 & 82.8 & \textbf{83.1}  & 79.2                                                                      & \multicolumn{1}{r}{\textbf{80.7}} & \textbf{77.6}                                                             & \multicolumn{1}{r}{75.4}          & \textbf{79.8}                                                             & \multicolumn{1}{r}{78.7}                         \\ \midrule
bc5cdr                                                                           & 90.0                                                                                                                                                  & \multicolumn{1}{r}{{90.4}} & 90.7                                                                                                                                                  & \multicolumn{1}{r}{{91.3}} & 91.3 & 91.8 & 90.7 & 89.9 & {87.8}                                                             & \multicolumn{1}{r}{87.5}          & 85.9                                                                      & \multicolumn{1}{r}{{88.3}} & 88.3                                                                      & \multicolumn{1}{r}{88.7}                \\
JNLPBA                                                                            & {79.4}                                                                                                                                         & \multicolumn{1}{r}{78.7}          & 78.8                                                                                                                                         & \multicolumn{1}{r}{79.0}  & 78.5 & 78.2 & 79.6 & 80.0 & {77.3}                                                             & \multicolumn{1}{r}{76.9}          & 74.0                                                                      & \multicolumn{1}{r}{{77.2}} & {78.6}                                                             & \multicolumn{1}{r}{78.5}                         \\
NCBI-disease                                                                       & 93.0                                                                                                                                                 & \multicolumn{1}{r}{{93.2}} & {93.4}                                                                                                                                        & \multicolumn{1}{r}{92.9}   & 93.3 & 93.4 & 92.8 & 93.5 & 91.1                                                                      & \multicolumn{1}{r}{{92.1}} & 89.9                                                                      & \multicolumn{1}{r}{{91.7}} & 90.5                                                                      & \multicolumn{1}{r}{91.3}                \\ \hdashline[1pt/1pt]
NER Avg.                & \textbf{87.5}                                                                                                                                         & \multicolumn{1}{r}{87.4}          & \textbf{87.7}                                                                                                                                         & \multicolumn{1}{r}{\textbf{87.7}} & 87.7 & \textbf{87.8} & 87.7 & \textbf{87.8}  & 85.4                                                                      & \multicolumn{1}{r}{\textbf{85.5}} & 83.3                                                                      & \multicolumn{1}{r}{\textbf{85.7}} & 85.8                                                                      & \multicolumn{1}{r}{\textbf{86.2}}     \\ \midrule
TriviaQA                                                          & 78.2                                                                                                                                                  & \multicolumn{1}{r}{{79.8}}  & 67.4                                                                                                                                                  & \multicolumn{1}{r}{{69.1}} & 80.6 & 81.8 & 77.4 & 78.2 & 72.2                                                                      & \multicolumn{1}{r}{{73.8}} & 69.2                                                                      & \multicolumn{1}{r}{{71.0}} & 64.7                                                                      & \multicolumn{1}{r}{66.8}                \\
SQuAD                                                             & 91.8                                                                                                                                                  & \multicolumn{1}{r}{{93.6}} & 87.5                                                                                                                                                 & \multicolumn{1}{r}{{88.5}} & 94.5 & 94.6 & 93.7 & 93.9 & 85.0                                                                      & \multicolumn{1}{r}{{87.0}} & 89.0                                                                      & \multicolumn{1}{r}{{89.6}} & 84.8                                                                      & \multicolumn{1}{r}{85.4}                \\ \hdashline[1pt/1pt]
\begin{tabular}[c]{@{}l@{}}QA Avg.\end{tabular} & 85.0                                                                                                                                                    & \multicolumn{1}{r}{\textbf{86.7}}  & 77.5                                                                                                                                                  & \multicolumn{1}{r}{\textbf{78.8}}  & 87.5 & \textbf{88.2} & 85.5 & \textbf{85.9} & 78.6                                                                      & \multicolumn{1}{r}{\textbf{80.4}} & 79.1                                                                      & \multicolumn{1}{r}{\textbf{80.3}} & 74.8                                                                      & \multicolumn{1}{r}{\textbf{76.1}} \\ \bottomrule          
\end{tabular}
\caption{Test scores of reduced (Rdc) models on the text classification, NER, and QA tasks. \textbf{Bold} indicates the best average score between the reduced and fully fine-tuned (Full) versions of each model. Each score represents the average macro F-1 score of 10 runs for RoBERTa, BERT, and the distilled models. The F-1 score averages for DeBERTa and T5 were gathered from 5 runs.
The standard errors for each score are shown in corresponding tables in \autoref{sec:experimental_setup}.  %in \autoref{tab:roberta}, \autoref{tab:bert}, \autoref{tab:distilbert}, \autoref{tab:minilm_768}, and \autoref{tab:minilm_384}.
For the ChemProt dataset, we report the micro F-1 scores instead, following past work \citep{beltagy2019scibert}. The reduced BERT-sized models generally offer similar performance to their full counterparts (scoring within 0.2\% when averaged across RoBERTa and SciBERT for the six tasks), and substantially outperform the distilled models. For the QA datasets, we use BERT while we use SciBERT for the text classification and NER datasets since it outperforms BERT on these datasets \citep{beltagy2019scibert}. The reduced models yield a small accuracy drop for QA tasks.
%For the reduced configurations, the half of the transformer layers closest to the input were frozen from fine-tuning. For adapters configurations (Frz+Adpt), we froze all the transformer layers from fine-tuning but added trainable adapters \cite{houlsby2019parameter} to the latter half of the transformer layers furthest from the input.
}
\label{tab:metatable}
\end{table*}














%\begin{table*}[ht]
%\centering
%\small
%\setlength{\tabcolsep}{6.0pt}
%\renewcommand{\arraystretch}{1.1}
%\begin{tabular}{@{}lrrrrrrrrrrrrrr@{}}
%\toprule
%                                                                           & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}RoBERTa \\ Large\end{tabular}}                                                                                                             & \multicolumn{2}{c}{BERT} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}DeBERTa \\ V2 XL \end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}T5 \\ Large\end{tabular}}                                                                                                                                                               & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}MiniLM\\ L6-H768\end{tabular}}                          & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}MiniLM\\ L6-H384\end{tabular}}                          & \multicolumn{2}{c}{DistilBERT}                                                               \\ \cmidrule(l{7pt}r{7pt}){2-3} \cmidrule(l{7pt}r{7pt}){4-5} \cmidrule(l{7pt}r{7pt}){6-7} \cmidrule(l{7pt}r{7pt}){8-9} \cmidrule(l{7pt}r{7pt}){10-11}
%                                   \cmidrule(l{7pt}r{7pt}){12-13}
%                                   \cmidrule(l{7pt}r{7pt}){14-15}
                                                                           
%Task                                                              & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}       & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}}      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Rdc\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Full\end{tabular}} \\ \midrule
%TriviaQA                                                          & 78.2                                                                                                                                                  & \multicolumn{1}{r}{{79.8}}  & 67.4                                                                                                                                                  & \multicolumn{1}{r}{{69.1}} & 80.6 & 81.8 & 93.3 & 93.7 & 72.2                                                                      & \multicolumn{1}{r}{{73.8}} & 69.2                                                                      & \multicolumn{1}{r}{{71.0}} & 64.7                                                                      & \multicolumn{1}{r}{66.8}                \\
%SQuAD                                                             & 91.8                                                                                                                                                  & \multicolumn{1}{r}{{93.6}} & 87.5                                                                                                                                                 & \multicolumn{1}{r}{{88.5}} & 94.5 & 94.6 & 93.7 & 93.9 & 85.0                                                                      & \multicolumn{1}{r}{{87.0}} & 89.0                                                                      & \multicolumn{1}{r}{{89.6}} & 84.8                                                                      & \multicolumn{1}{r}{85.4}                \\ \hdashline[1pt/1pt]
%\begin{tabular}[c]{@{}l@{}}QA Avg.\end{tabular} & 85.0                                                                                                                                                    & \multicolumn{1}{r}{\textbf{86.7}}  & 77.5                                                                                                                                                  & \multicolumn{1}{r}{\textbf{78.8}}  & 87.5 & 88.2 & 93.5 & 93.8 & 78.6                                                                      & \multicolumn{1}{r}{\textbf{80.4}} & 79.1                                                                      & \multicolumn{1}{r}{\textbf{80.3}} & 74.8                                                                      & \multicolumn{1}{r}{\textbf{76.1}} \\ \bottomrule              
%\end{tabular}
%\caption{Test scores of reduced (Rdc) models on the QA tasks. \textbf{Bold} indicates the best average score between the reduced and fully fine-tuned (Full) versions of each model. Each score represents the average macro F-1 score of 10 runs, with the standard errors for each score in \autoref{sec:experimental_setup}.  The reduced models yield a small accuracy drop for QA tasks.%\autoref{tab:roberta}, \autoref{tab:bert}, \autoref{tab:distilbert}, \autoref{tab:minilm_768}, and \autoref{tab:minilm_384}. %For the reduced (Rdc) configurations, the earlier half of the transformer layers closest to the input were frozen from fine-tuning.}
%}
%\label{tab:qa_results}
%\end{table*}
